Minimizing Completion Times for Stochastic Jobs via Batched Free Times

We study the classic problem of minimizing the expected total completion time of jobs on $m$ identical machines in the setting where the sizes of the jobs are stochastic. Specifically, the size of each job is a random variable whose distribution is known to the algorithm, but whose realization is revealed only after the job is scheduled. While minimizing the total completion time is easy in the deterministic setting, the stochastic problem has long been notorious: all known algorithms have approximation ratios that either depend on the variances, or depend linearly on the number of machines. We give an $\widetilde{O}(\sqrt{m})$-approximation for stochastic jobs which have Bernoulli processing times. This is the first approximation for this problem that is both independent of the variance in the job sizes, and is sublinear in the number of machines $m$. Our algorithm is based on a novel reduction from minimizing the total completion time to a natural makespan-like objective, which we call the weighted free time. We hope this free time objective will be useful in further improvements to this problem, as well as other stochastic scheduling problems.

==> anupam.tex <==

\newpage

\section{Anupam's Notes}

Here are three problems:
\begin{enumerate}[(a)]
\item The original scheduling problem (sumCj): Given a set of jobs,
  minimize $\sum_j C_j$. We compare to $Opt$, which is the optimal
  minimum total completion time of an adaptive non-clairvoyant policy
  
\item Nested Subset Selection Problem (NSS): choose nested sets of jobs
  $J_1 \sse J_2 \sse $ such that $|J_i| \approx n(1-\frac{L}{2^i})$
  and moreover ``the jobs in $J_k$ are better than OPT's first
  $n(1-1/2^k)$ jobs'', ideally they are a subset of OPT's first jobs
  in every realization, which is what happens in Bernoulli jobs. But
  maybe some kind of inequality like
  \begin{gather}
    \EE[ \tilde{F}^*(J_k) ] \leq \beta \cdot \EE[ F^{Opt}(n(1-1/2^k))
    ] \label{eq:todo}
  \end{gather}
   for all $k$ simultaneously, which is the crucial inequality
  in the proof of Thm 3.4. Here the LHS is the optimal free time of
  the set $J_k$ under this batching constraint, and the RHS is the
  optimal free time of the first $n(1-1/2^k))$ jobs without batching
  constarints.
  
\item The Batched Free Time Minimization Problem (BFT). This one just
  says: find an ordering such that for all $k$ simultaneously,
  \[ \EE[ \tilde{F}(J_k) ] \leq \alpha \EE[ \tilde{F}^*(J_k) ] , \]
  where the LHS is the free time of the algorithm under the batching,
  the RHS is the that of the optimal schedule also under the batching.
\end{enumerate}

And here are the facts:
\begin{enumerate}[i.]
\item We know how to solve BFT for general job sizes. (Check!)
  $\alpha$ is constant for Bernoullis, and $O(\log m)$ for general
  sizes, I think.
 
\item Thm 3.4 shows that if we can solve NSS and BFT for some class of
  jobs, then we get an $O(\alpha \beta L)$ for SumCj for that
  class. This means we really need to understand NSS.

\item The hand-written writeup proves a weaker version of
  (\ref{eq:todo}) for general jobs: it considers a single batch (just
  $J_1$), and shows this inequality with the optimal \emph{list
    schedule} on the right. So we would need to (a) extend to general
  adaptive OPT for this FT-minimization problem, and (b) then show it
  for multiple batches. These are two missing pieces of the puzzle.
   
\end{enumerate}

To recap, the things we have to prove are:

\begin{enumerate}
    \item Prove (1) for deterministic jobs, then for Bernoulli jobs, then for general jobs. 
    \item Prove that given a set of stochastic jobs, if job $j_1$ stochastic dominates $j_2$ then the optimal adaptive policy always does $j_1$ before $j_2$. This we have shown for Bernoulli jobs (we think, and Rudy is writing/checking the details \alert{see \Cref{lem_sortprob} for Bernoulli case}), and need to show for general jobs. (cf. the Weber et al.\ paper, which shows this for jobs where the stochastic domination property gives a total order, and not just a partial order).
    \item Show that sizes etc can be poly-bounded. \alert{see \Cref{lem_bernoilli_rescale} for Bernoulli case and Ben's paper for general}
\end{enumerate}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> batch_free_time_general.tex <==
\section{Batch Free Time Minimization for General Distributions}\label{sec_batch_free_time_general}

In this section we solve Batch Free Time Minimization for general job distributions. We begin with a reduction from BFT to free time minimization (for a single set of jobs.) The proof is analogous to \Cref{thm_warmreduce}.

\begin{theorem}\label{thm_ft_to_bft}
    Suppose there exists an efficient algorithm that outputs a $\alpha$-approximate list schedule for free time minimization. There there exists an efficient algorithm that outputs a $(\alpha + 1)$-approximate list schedule for BFT. Further, if the algorithm for free time minimization is approximate on a per-realization basis, then the resulting BFT algorithm is as well.
\end{theorem}
\begin{proof}
    Let $\mathcal{A}$ be the algorithm for free time minimization guaranteed by the theorem. Our algorithm for BFT is the following. For each batch $k = 1, \dots, K$, we run $\mathcal{A}$ on $J_k \setminus J_{k-1}$ to obtain a list schedule of $J_k \setminus J_{k-1}$. Then, we output the concatenation of this lists $J_1, J_2 \setminus J_1, \dots, J_K \setminus J_{K-1}$.
    
    This algorithm is clearly efficient and outputs a list schedule because $\mathcal{A}$ does as well. Further, the algorithm satisfies the batch constraint. It remains to show that it is $(\alpha + 1)$-approximate for BFT. We do so by induction of $k$. In particular, we show by induction on $k$ that $\mathbb{E} \tilde{F}(J_k) \leq (\alpha + 1) \mathbb{E} (\tilde{F}^*(J_1) + \cdots + \tilde{F}^*(J_k))$ for all $k =1, \dots, K$. Further, if $\mathcal{A}$ is a per-realization approximation, then $\tilde{F}_r(J_k) \leq (\alpha + 1) (\tilde{F}^*_r(J_1) + \cdots + \tilde{F}^*_r(J_k))$ for every realization $r$ of job sizes. The subscript $r$ denotes that we condition on realization $r$.
	
	The base case $k = 1$ is immediate because $\mathcal{A}$ is a $\alpha$-approximation for free time minimization.
	
	Now we consider the inductive case $k > 1$. Condition on any realization of job sizes $r$. For this inductive step, we say a job is \emph{big} if its realized size is strictly greater than $\tilde{F}^*_r(J_k)$ and \emph{small} otherwise. Now consider the optimal schedule of $J_k$ subject to the batch constraints achieving free time $\tilde{F}^*_r(J_k)$.
	
	We claim that there are strictly less than $m$ big jobs in $J_{k-1}$. Suppose not. By definition of big, Opt can schedule at most one big job per machine to achieve free time $\tilde{F}^*_r(J_k)$. However, there are at least $m$ big jobs by assumption, so Opt must schedule at least one per machine. This contradicts the optimal free time.
	
	Now we relate the initial loads that our algorithm and Opt experience when scheduling $J_k \setminus J_{k-1}$ after $J_{k-1}$. We define $m' = m - \#\{\text{big jobs in $J_{k-1}$}\}$. By the previous claim, $m' > 0$. Now consider Opt scheduling $J_k \setminus J_{k-1}$ after $J_{k-1}$. Any machine that already started a big job from $J_{k-1}$ is not used to schedule any job in $J_k \setminus J_{k-1}$. Further, Opt scheduled each big job on a separate machine, so the optimal schedule schedules $J_k \setminus J_{k-1}$ on $m'$ machines each with initial load at least $\tilde{F}^*_r(J_{k-1})$.
	
	On the other hand, for our algorithm, consider time $\tilde{F}_r(J_{k-1})$. At this time, all jobs in $J_{k-1}$ are finished or currently in progress. In particular, at least $m'$ machines are free or scheduling small jobs. These machines can start $J_k \setminus J_{k-1}$ by time $\tilde{F}_r(J_{k-1}) + \tilde{F}^*_r(J_k)$. Thus, our algorithm schedules $J_k \setminus J_{k-1}$ on at least $m'$ machines each with initial load at most $\tilde{F}_r(J_{k-1}) + \tilde{F}^*_r(J_k)$.

	Using \Cref{lem_listprop}, we can bound $\tilde{F}_r(J_k)$ with respect to $F_r(J_k \setminus J_{k-1})$ and our algorithm's initial load. Recall that our algorithm schedules $J_k \setminus J_{k-1}$ on at least $m'$ machines with initial loads at most $\tilde{F}_r(J_{k-1}) + \tilde{F}^*_r(J_k)$. However, decreasing the number of machines to $m'$ and increasing their initial loads to $\tilde{F}_r(J_{k-1}) + \tilde{F}^*_r(J_k)$ can only increase the free time by the lemma. Thus:
	\begin{equation}\label{eq_alg_batch_upper}
	    \tilde{F}_r(J_k) \leq (\tilde{F}_r(J_{k-1}) + \tilde{F}^*_r(J_k)) + F_r(J_k \setminus J_{k-1}, m'),
	\end{equation}
	where $F_r(J_k \setminus J_{k-1}, m')$ is defined to be the free time with $m'$ machines (as opposed to the initial $m$.)
	
	We lower bound $\tilde{F}^*_r(J_k)$ similarly with respect to $F^*_r(J_k \setminus J_{k-1})$ and Opt's initial load. We recall that Opt schedules $J_k \setminus J_{k-1}$ on at most $m'$ machines with initial loads at least $\tilde{F}^*_r(J_{k-1})$. Then we can lower bound:
	\begin{equation}\label{eq_opt_batch_lower}
	    \tilde{F}^*_r(J_k) \geq \tilde{F}^*_r(J_{k-1}) + F_r^*(J_k \setminus J_{k-1}, m').
	\end{equation}
	
	To complete the proof, we first show the BFT guarantee holds in expectation, and then per-realization (if $\mathcal{A}$ is also per-realization.) We may assume inductively that $\mathbb{E} \tilde{F}(J_{k-1}) \leq (\alpha + 1) \mathbb{E} (\tilde{F}^*(J_1) + \cdots + \tilde{F}^*(J_{k-1}))$. Further, the properties of $\mathcal{A}$ give $\mathbb{E} F(J_k \setminus J_{k-1}, m') \leq \alpha \mathbb{E} F^*(J_k \setminus J_{k-1}, m')$. Taking expectations with respect to the random realization $r$ and applying the above two inequalities to \Cref{eq_alg_batch_upper} gives:
	\[ \mathbb{E} \tilde{F}(J_k) \leq (\alpha + 1)\mathbb{E} (\tilde{F}^*(J_1) + \cdots + \tilde{F}^*(J_{k-1})) + \mathbb{E} \tilde{F}^*(J_k) + \alpha \mathbb{E} F^*(J_k \setminus J_{k-1}, m').\]
	Similarly, taking expectations in \Cref{eq_opt_batch_lower} and combining with the above upper-bound give the desired inequality.
	
	The proof of the per-realization guarantee is analogous by applying the stronger inductive hypothesis $\tilde{F}_r(J_{k-1}) \leq (\alpha + 1) (\tilde{F}^*_r(J_1) + \cdots + \tilde{F}^*_r(J_{k-1}))$ and $\mathcal{A}$'s guarantee $F_r(J_k \setminus J_{k-1}, m') \leq \alpha F^*_r(J_k \setminus J_{k-1}, m').$
\end{proof}

It remains to give an algorithm for free time minimization for general job distributions. This is our random list schedule.

\begin{theorem}[Random List Schedule]\label{thm_random_list_free}
    List scheduling jobs in uniformly random order is a $O(\log m)$-approximation in expectation for free time minimization per-realization (i.e. conditioned on any realization of job sizes and then taking expectation over only the randomness of the algorithm, this algorithm is $O( \log m)$-approximate.)
\end{theorem}
\begin{proof}
    It suffices to prove the theorem for \emph{deterministic jobs}, because for general job distributions we can condition on any realization. Thus, let $J$ be a set of deterministic jobs with sizes $s_j$ for all $j \in J$ and $Opt$ the optimal free time of $J$. For this proof, a job is \emph{big} if its size is larger than $Opt$ and \emph{small} otherwise. Let $b$ denote the number of big jobs. Then by definition of $Opt$, we have $b < m$.
    
    First, we consider any fixed list schedule of $J$. We can partition the small jobs into sets $S_0, \dots, S_b$, where $S_i$ is the set of all small jobs started between the $i$th and $(i+1)$st big jobs started. Thus, the order we schedule is $S_0$, first big job, $S_1$, second big job, and so on. Note that when we start $S_i$, we have already scheduled $i$ big jobs, so we have at least $m - i$ machines which have not yet scheduled any big job.
    
    For $i = 0, \dots, b$, we define $V_i$ to be the total load of the machines \emph{with no big jobs} after scheduling $S_i$ (not including the $(i+1)$st big job.) The free time of our list schedule is the load of the least-loaded machine after scheduling $S_b$. By averaging over the at least $m-b$ machines with no big jobs, we can upper bound the free time by $\frac{1}{m-b} V_b$. Thus, it remains to upper bound $V_b$ in terms of $Opt$. We achieve this by an iterative volume argument in the next lemma. For  $J' \subset J$, let $Vol(J') = \sum_{j \in J'} s_j$ be the total size of all jobs in $J'$.
    
    \begin{lem}\label{lem_iter_vol}
        For all $i = 0, \dots b$, we have $V_i \leq (m-i) (\sum_{k = 0}^i \frac{1}{m-k} Vol(S_k) + \sum_{k = 1}^i \frac{1}{m - k} Opt)$.
    \end{lem}
    \begin{proof}
        We do induction on $i = 0, \dots b$. In the base case $i = 0$, we have $V_0 = Vol(S_0)$, because no machine has scheduled a big job yet.
        
        In the inductive case $i > 0$, let $V'$ denote the total load of the machines with no big jobs after scheduling $S_{i-1}$ and the subsequent big job. Then we have:
        \[V_i \leq V' + Vol(S_i),\]
        so it remains to upper bound $V'$. To obtain $V'$ from $V_{i-1}$, we remove the load of the least-loaded machine with no big job from $V_{i-1}$. In $V_{i-1}$, we have at least $m - i + 1$ machines with no big jobs. These machines have loads within $\pm Opt$ of each other, because they have only scheduled small jobs. In particular, by averaging, the load of the least-loaded such machine is at least $\frac{1}{m - i + 1} V_{i-1} - Opt$. Thus we can upper bound:
        \[V' \leq V_{i-1} - (\frac{1}{m - i + 1} V_{i-1} - Opt) = \frac{m-i}{m-i+1} V_{i - 1} + Opt.\]
        Plugging in this upper bound for $V'$ into our expression for $V_i$ and then applying the inductive hypothesis to $V_{i-1}$ gives the desired inequality.
    \end{proof}
    
    In particular, the above lemma gives:
    \[\frac{1}{m-b} V_b \leq \sum_{k = 0}^b \frac{1}{m-k} Vol(S_k) + \sum_{k = 1}^b \frac{1}{m - k} Opt \leq \sum_{k = 0}^b \frac{1}{m-k} Vol(S_k) + O(\log m) Opt.\]
    Now we consider a random list schedule. Let $Alg$ be a random variable denoting the free time achieved by the random list schedule. Now, the sets $S_0, \dots, S_b$ and subsequently the quantities $V_0, \dots, V_b$ are random. Taking expectations and applying the above inequality:
    \[\mathbb{E} Alg \leq \mathbb{E} \frac{1}{m-b} V_b \leq \sum_{k = 0}^b \frac{1}{m-k} \mathbb{E} Vol(S_k) + O(\log m) Opt.\]
    It remains to show $\sum_{k = 0}^b \frac{1}{m-k} \mathbb{E} Vol(S_k) = O(\log m) Opt$. Let $S \subset J$ be the set of all small jobs. Then by linearity of expectation, $\mathbb{E} Vol(S_k) = \frac{1}{b+1} Vol(S)$, because there are $b+1$ sets $S_0, \dots, S_b$, so every small job ends up in $S_k$ with probability $\frac{1}{b+1}$. Thus we can re-write:
    \[\sum_{k = 0}^b \frac{1}{m-k} \mathbb{E} Vol(S_k) = \frac{Vol(S)}{b+1} \sum_{k = 0}^b \frac{1}{m-k}.\]
    Now we lower bound $Opt$ in terms of $Vol(S)$.  
    
    \begin{lem}\label{lem_opt_small_lower}
        We have $Opt \geq \frac{1}{2} \frac{Vol(S)}{m}$.
    \end{lem}
    \begin{proof}
        We lower bound $Opt$ by the optimal free time on the instance of only small jobs. The free time of this sub-instance is the load of the least-loaded machine, which by averaging is at least $\frac{Vol(S)}{m} - Opt$. We conclude, $Opt \geq \frac{Vol(S)}{m} - Opt$.
    \end{proof}
    
    To complete the proof, we combine the above lemma with our expression for $\sum_{k = 0}^b \frac{1}{m-k} \mathbb{E} Vol(S_k)$:
    \[\sum_{k = 0}^b \frac{1}{m-k} \mathbb{E} Vol(S_k) = \frac{Vol(S)}{m} \frac{m}{b + 1} \sum_{k = 0}^b \frac{1}{m-k} \leq \frac{Vol(S)}{m} \sum_{k = 0}^b \frac{1}{b + 1 - k} = O(\log m) Opt,\]
    where we use the fact that $\frac{m}{b +1} \frac{1}{m-k} \leq \frac{1}{b + 1 - k}$ for all $k = 0, \dots, b$ (because $b \leq m -1$.)
\end{proof}


==> choose_jobs.tex <==
\section{Approximating Free Times for Bernoulli Jobs}\label{sec_choose_jobs}

The previous section holds for minimizing completion time of stochastic jobs on identical machines. In particular, the results do not rely on Bernoulli jobs. From now on, we will consider instances with only Bernoulli jobs. Our results will be parametrized by the number of distinct Bernoulli sizes, which we denote by $L$. Later, we show by standard rescaling and discretization techniques that we may assume $L = O(\log n)$ and lose only an extra constant factor in our final approximation ratio.

The goal of this section is to minimize the quantity $\sum_{k = 1}^{\log n} n/2^k F(n - n/2^k)$. We recall that our final algorithm will be a \emph{list schedule}. We let $F^*(i)$ denote the $i$th free time achieved by the optimal schedule that minimizes the completion time. We will split our algorithm design into two main parts:

First, for each $k$, we choose a set of (approximately) $n-n/2^k$ jobs that our list schedule will start first such that our jobs are comparable to the first $n-n/2^k$ jobs of the optimal schedule. We note that the optimal schedule is adaptive, so the first $n-n/2^k$ jobs the optimal schedule decides to start is not a fixed set of jobs in general. In contrast, the first $n-n/2^k$ jobs of our list schedule is fixed.

Second, after deciding these sets of jobs, we need to determine an ordering on these jobs such that our free times are comparable with the optimal free times.

\subsection{Choosing Sets of Jobs}

For the moment, we focus on choosing a set of jobs that are comparable to the first $n - n/2^k$ jobs of the optimal schedule for a single $k$. Throughout this paper, we let $J_k^*$ be the random set consisting of the first $n - n/2^k$ jobs scheduled by the optimal completion time schedule. The key of our analysis is the following simple lower bound on the optimal schedule:

\begin{center}
	\it The optimal schedule can exclude only $n/2^k$ jobs from $J_k^*$.
\end{center}

It is convenient to think of the $n/2^k$ jobs that the optimal schedule \emph{excludes} from contributing to $F^*(n - n/2^k)$ rather than the jobs it chooses to start. Similarly, we choose the set of jobs for our algorithm also by its exclusions.

Recall that we consider Bernoulli jobs with $L$ distinct sizes. Using our lower bound, the optimal schedule can exclude at most $n/2^k$ jobs from each Bernoulli size. The next lemma characterizes what jobs the optimal chooses to exclude from each size. The proof is an exchange argument.

\begin{lem}\label{lem_sortprob}
	Let $J$ be a set of Bernoulli jobs. Then for each size, the optimal completion time schedule for $J$ starts the jobs of this size in increasing order of their probabilities for all realizations of the job sizes. \alert{to check and probably add picture}
\end{lem}
\begin{proof}
    We suppose there exist jobs $a,b$ such that $X_a \sim s \cdot Ber(p_a)$ and $X_b \sim s \cdot Ber(p_b)$ with $p_a \leq p_b$ such that the optimal completion time policy schedules $b$ before $a$ in some realization. We can represent this policy by a decision tree. Thus, we assume this tree schedules $b$ before $a$ is some realization (i.e. some root-leaf path.) It follows, there exists a subtree rooted at $b$ such that $a$ is scheduled on each root-leaf path of this subtree. We denote this subtree by $T$. Entering this subtree, the machines have some fixed initial loads and $T$ schedules a fixed set of jobs $J$.
    
    We will modify the subtree $T$ so that we start $a$ before $b$ on each root-leaf path. Further, this will not increase the expected completion time of the overall schedule. We construct the modified subtree $T'$ as follows. Let the left- and right subtrees (corresponding to the root job $b$ coming up size $0$ or $s$) of $T$ be $T_L$ and $T_R$, respectively. $T'$ is rooted at job $a$. The right subtree of $a$ is $T_R$, but with job $a$ replaced by job $b$. We denote this modifed subtree by $T_R(a \rightarrow b)$. On the left subtree of $a$, first, independently of all jobs, we flip a coin that comes up heads with probability $q$. We will choose $q$ later. If the coin is heads, then we schedule subtree $T_L$ with job $a$ replaced by job $b$, so $T_L(a \rightarrow b)$. Otherwise, if the coin is heads, then we schedule $b$. The left- and right subtrees of $b$ are $T_L$ and $T_R$, except the job $a$ is replaced by a dummy job that is always zero. In particular, this job does not contribute to the completion time, but upon reaching this node we will always follows the left subtree. We denote these subtrees by $T_L(-a), T_R(-a)$, respectively. This completes the description of $T'$.
    
    Note that $T'$ schedules the same jobs as $T$ and always starts $a$ before $b$. It remains to choose $q$ such that the expected completion time of $T'$ is the same as $T$. We choose $q$ such that the probability of entering $T_R(a \rightarrow b)$ or $T_R(-a)$ is exactly $p_b$. We conflate the name of a subtree (e.g. $T_R(a \rightarrow b)$) with the event that we enter the subtree. Thus, we want $\mathbb{P}(T_R(a \rightarrow b) \vee T_R(-a)) = p_b$. The former probability is exactly $p_a + \bar{p}_a q p_b$, where we define $\bar{p} = 1 - p$ for a probability $p$. This gives $q = \frac{p_b - p_a}{\bar{p}_a p_b}$. Thus, we have chosen $q$ such that $\mathbb{P}(T_R(a \rightarrow b) \vee T_R(-a)) = p_b$ and $\mathbb{P}(T_L(a \rightarrow b) \vee T_L(-a)) = \bar{p}_b$. One should imagine that these two events are our replacements for the original tree $T$ entering $T_R$ and $T_L$. 
    
    In both subtrees $T_L(a \rightarrow b)$ and $T_L(-a)$, we replace the original job $a$ from $T_L$ with $b$ and a zero job, respectively. Let $\tilde{X}_a$ denote the size of the the replacement job, which is supported on $\{0, s\}$. We compute the distribution of $\tilde{X}_a$:
    \[\mathbb{P}(\tilde{X}_a = s \mid T_L(a \rightarrow b) \vee T_L(-a)) = \frac{\mathbb{P}(T_L(a \rightarrow b))}{\mathbb{P}(T_L(a \rightarrow b) \vee T_L(-a))} p_b = \frac{\bar{p}_a \bar{q}}{\bar{p}_b} p_b = p_a.\]
    It follows, conditioned on $T_L(a \rightarrow b) \vee T_L(-a)$, our replacement job for $a$ has the same distribution as $a$. An analogous computation for the right subtree gives:
    \[\mathbb{P}(\tilde{X}_a = s \mid T_R(a \rightarrow b) \vee T_R(-a)) = \frac{\mathbb{P}(T_R(a \rightarrow b))}{\mathbb{P}(T_R(a \rightarrow b) \vee T_L(-a))} p_b = \frac{p_a}{p_b} p_b = p_a,\]
    so the distribution of our replacement job conditioned on $T_R(a \rightarrow b) \vee T_R(-a)$ has the same distribution as $a$ as well.
    
    To summarize, we have constructed a tree $T'$ that starts $a$ before $b$. $T'$ enters $T_L(a \rightarrow b)$ or $T_L(-a)$ with probability $\bar{p}_b$: exactly the same as the probability that $T$ enters $T_L$. Further, $T'$ enters $T_L(a \rightarrow b)$ or $T_L(-a)$ with the same initial loads as $T$ entering $T_L$, because both correspond to all previous jobs in the subtree having size $0$. Finally, upon entering $T_L(a \rightarrow b)$ or $T_L(-a)$, the job we replace $a$ with has the same distribution as $a$. The analogous properties hold for the right subtree as well. We conclude, for any job $j \in J \setminus \{a,b\}$, the expected completion time of $j$ in $T'$ is the same as in $T$ (subject to the same initial loads.)
    
    It remains to show that the expected completion time of $a$ and $b$ weakly decreases from $T$ to $T'$. We define $\ell' \sim T_L$ to be the load of the least-loaded machine upon reaching the node $a$ in subtree $T_L$ (we define $\ell' \sim T_R$ analogously.) This is well-defined, because $a$ is scheduled on every root-leaf path in $T_L$. Note that $\ell'$ does not depend on the job scheduled at node $a$. It follows, the expected completion time of $a$ and $b$ in $T'$ are:
    \[\mathbb{E}_{T'} \,C_a = \ell + s p_a\]
    \[\mathbb{E}_{T'} \,C_b = \mathbb{P}(T_L(a \rightarrow b)) (\mathbb{E}_{\ell' \sim T_L} \ell' + sp_b) + \mathbb{P}(T_L(-a)) \ell + \mathbb{P}(T_R(-a)) (\ell + s) + \mathbb{P}(T_R(a \rightarrow b)) (\mathbb{E}_{\ell' \sim T_R} \ell' + s p_b).\]
    Now we simplify the completion time of $b$. First, we consider the terms corresponding to the left subtree. We have $\mathbb{P}(T_L(a \rightarrow b)) = \bar{p}_b\frac{p_a}{p_b}$, $\mathbb{P}(T_L(a \rightarrow b)) + \mathbb{P}(T_L(-a)) = \bar{p}_b$, and $\ell' \geq \ell$ for $\ell' \sim T_L$. Combining these three observations:
    \begin{align*}
        \mathbb{P}(T_L(a \rightarrow b)) (\mathbb{E}_{\ell' \sim T_L} \ell' + sp_b) + \mathbb{P}(T_L(-a)) \ell &= \mathbb{P}(T_L(a \rightarrow b)) \mathbb{E}_{\ell' \sim T_L} \ell' + \bar{p}_b s p_a + \mathbb{P}(T_L(-a)) \ell\\
        &\leq \bar{p}_b (\mathbb{E}_{\ell' \sim T_L} \ell' + s p_a).
    \end{align*}
    Now we consider the right subtree. Analogously, we have $\mathbb{P}(T_R(a \rightarrow b)) = p_a$, $\mathbb{P}(T_R(a \rightarrow b)) + \mathbb{P}(T_R(-a)) = p_b$, and $\ell' \geq \ell$ for $\ell' \sim T_R$. We compute:
    \begin{align*}
        \mathbb{P}(T_R(-a)) (\ell + s) + \mathbb{P}(T_R(a \rightarrow b)) (\mathbb{E}_{\ell' \sim T_R} \ell' + s p_b) &= (p_b - p_a) (\ell + s) + p_a \mathbb{E}_{\ell' \sim T_R} \ell' + s p_b + p_a s p_b\\
        &\leq p_b (\mathbb{E}_{\ell' \sim T_R} \ell' + p_a s) + (p_b - p_a) s.
    \end{align*}
    Combining our expressions for the left- and right-subtrees gives our final bound on the completion time of $a$ and $b$:
    \[\mathbb{E}_{T'} \,C_a + \mathbb{E}_{T'} \,C_b \leq \ell + s p_b + \bar{p}_b (\mathbb{E}_{\ell' \sim T_L} \ell' + s p_a) + p_b (\mathbb{E}_{\ell' \sim T_R} \ell' + p_a s) = \mathbb{E}_T \,C_b + \mathbb{E}_T \,C_a.\]
\end{proof}

On the other hand, our algorithm will exclude $n/2^k$ jobs of each Bernoulli size simultaneously. The lemma suggests that we might as well exclude the jobs with largest $p_j$'s. In particular, our algorithm to choose sets of jobs that are comparable to the $J_k^*$'s is the following:

\choosealg: For each $k = 1, \dots, \log n$, let $J_k$ be the set of jobs constructed as follows:
    	\begin{itemize}
    		\item Initialize $J_k = J$.
    		\item For each Bernoulli size $s$, remove from $J_k$ the $n/2^k$ jobs of size $s$ with largest $p_j$'s.
    		\item Output $J_k$.
    	\end{itemize}

The $J_k$-sets are comparable to the first $n - n/2^k$ jobs of the optimal schedule in the following sense:

\begin{lem}\label{lem_batch_prefix}
    The $J_k$'s output by \choosealg satisfy:
    \begin{itemize}
        \item $J_1 \subset \dots \subset J_{\log n} \subset J$
    	\item $\lvert J_k \rvert \in [n - L \cdot n/2^k, n - n/2^k]$
        \item $J_k \subset J_k^*$ for all $k$ and all realizations.
    \end{itemize}
\end{lem}
\begin{proof}
    	It is immediate that the sets $J_1, \dots, J_{\log n}$ are nested and have the desired size. It remains to show that $J_k \subset J_k^*$. Note that Opt excludes at most $n/2^k$ jobs of the largest probabilities of each size by \Cref{lem_sortprob}. This holds for all realizations. On the other hand, we exclude $n/2^k$ jobs of largest probability of all sizes simultaneously.
\end{proof}

\begin{comment}
    The next theorem formalizes this idea.


    \begin{theorem}\label{thm_choosejobs}
    	Let $J$ be a set of $n$ Bernoulli jobs with $L$ distinct sizes. There exists an efficient algorithm that outputs nested sets of jobs $J_1 \subset \dots \subset J_{\log n} \subset J$ such that for all $k$:
    	\begin{enumerate}
    		\item $\lvert J_k \rvert \in [n - L \cdot n/2^k, n - n/2^k]$
    		\item $J_k$ is a subset of the first $n-n/2^k$ jobs started by the optimal completion time schedule for all realizations.
    	\end{enumerate}
    \end{theorem}
    \begin{proof}
    	For each $k$, we construct $J_k$ with the following algorithm:
    	
    	\begin{itemize}
    		\item Initialize $J_k = J$.
    		\item For each Bernoulli size $s$, remove from $J_k$ the $n/2^k$ jobs of size $s$ with largest $p_j$'s.
    		\item Output $J_k$.
    	\end{itemize}
    	
    	It is immediate that the sets $J_1, \dots, J_{\log n}$ are nested and have the desired size. It remains to show that $J_k$ is a subset of the first $n-n/2^k$ jobs of Opt. Note that Opt excludes at most $n/2^k$ jobs of the largest probabilities of each size by \Cref{lem_sortprob}. This holds for all realizations. On the other hand, we exclude $n/2^k$ jobs of largest probability of all sizes simultaneously.
    \end{proof}
\end{comment}

Morally, \Cref{lem_batch_prefix} states that we ``know" the jobs that Opt starts to achieve $F^*(n-n/2^k)$ for all $k$ (up to a $L$-factor.) This suggests that we should first schedule $J_1$ to get free time comparable to $F^*(n-n/2^1)$, and then $J_2 \setminus J_1$ to get free time comparable to $F^*(n-n/2^2)$, and so on. Before considering this problem algorithmically, we first show that there exists a good list schedule of the $J_k$'s satisfying this \emph{batch constraint} (we must start all jobs in $J_{k-1}$ before any job in $J_k \setminus J_{k-1}$ for all $k$.) Note that in general, even though $J_k \subset J_k^*$ for all $k$, it is not the case that the optimal completion time schedule satisfies the batch constraint. \alert{should say some stuff about why this is the hardest part of our work}

\begin{theorem}\label{thm_batches_opt_cost}
    The $J_k$'s output by \choosealg satisfy:
    \[\sum_{k =1}^{\log n} n/2^k \cdot \mathbb{E} \tilde{F}^*(J_k) = O(\sqrt{m} \cdot poly(\log n)) (\sum_{k =1}^{\log n} n/2^k \cdot \mathbb{E} F^*(n-n/2^k) + \sum_j \mathbb{E} C_j^*),\]
    where $\tilde{F}^*(J_k)$ is the optimal free time of $J_k$ subject to the batch constraint.
\end{theorem}

The proof of \Cref{thm_batches_opt_cost} is one of the main technical contributions of this work. Before proving the theorem, we first use it to give the $O(\sqrt{m} \cdot poly(\log n))$-approximate algorithm guaranteed by \Cref{thm_mainber}. In particular, it remains to algorithmically find a good list schedule of the $J_k$'s satisfying the batch constraint.

\subsection{Ordering the Jobs}

Now suppose we run \choosealg to obtain jobs $J_1 \subset \dots \subset J_{\log n} \subset J$. To construct a list schedule with these sets, we start all jobs in $J_1$, then $J_2 \setminus J_1$, and so on.\footnote{Note that $J_{\log n} \neq J$ in general, so this procedure leaves some jobs unscheduled. There are only $O(L)$ such unscheduled jobs, which we will deal with later.}

However, it remains to decide what order to schedule the jobs within $J_k \setminus J_{k-1}$ for each $k$. To this end, we define the following (artificial) scheduling problem.

\begin{definition}[Batch Free Time Minimization]
	Given nested sets of stochastic jobs, $J_1 \subset \dots \subset J_K$, we want to construct a \emph{list schedule} of $J_K$ subject to the constraint that we must start all jobs in $J_{k-1}$ before any job in $J_k \setminus J_{k-1}$ for all $k$. The goal is to guarantee that $\mathbb{E} \tilde{F}(J_k) \leq \alpha (\mathbb{E} \tilde{F}^*(J_1) + \cdots + \mathbb{E} \tilde{F}^*(J_k))$ for all $k$ simultaneously and some $\alpha \geq 1$, where $\tilde{F}(J_k)$ is free time of $J_k$ achieved by our algorithm, and $\tilde{F}^*(J_k)$ is analogous optimal free time (subject to the same constraint.)
\end{definition}

In light of \Cref{thm_batches_opt_cost}, we can reduce minimizing completion time to solving batch free time minimization.

\begin{theorem}\label{thm_batchreduce}
	Suppose there exists an efficient algorithm for Batch Free Time Minimization for Bernoulli jobs with $L$ sizes. Then there exists an efficient $O(\alpha L \sqrt{m} \cdot poly(\log n))$-approximation for minimizing the completion time of Bernoulli jobs with $L$ sizes.
\end{theorem}
\begin{proof}
	Our algorithm is the following:
	\begin{itemize}
		\item On input Bernoulli jobs $J$, run \choosealg to obtain sets of jobs $J_1 \subset \dots \subset J_{\log n}$.
		\item On the nested jobs $J_1 \subset \dots \subset J_{\log n}$, run the algorithm assumed by the theorem statement to obtain a list schedule of $J_{\log n}$.
		\item Output the final list scheduling consisting of the list schedule on $J_{\log n}$ and then the remaining jobs $J \setminus J_{\log n}$ in arbitrary order.
	\end{itemize}

	By definition of the assumed algorithm, we have $\mathbb{E} \tilde{F}(J_k) \leq \alpha (\mathbb{E} \tilde{F}^*(J_1 ) + \cdots + \mathbb{E} \tilde{F}^*(J_k))$ for all $k$.
	
	To complete the proof, we bound the expected completion time of our list schedule with respect to $Opt$, the optimal expected completion time. First, we deal with the jobs in $J \setminus J_{\log n}$. By \Cref{lem_batch_prefix}, $\lvert J \setminus J_{\log n} \rvert = O(L)$. Further, by Graham's list schedule, any list schedule of $J$ is $2$-approximate for makespan on a per-realization basis. In particular, in expectation the completion time of each job in $J \setminus J_{\log n}$ is upper-bounded by $O(1)$ times the optimal expected makespan, which is a lower bound on the optimal expected completion time. To summarize, the jobs in $J \setminus J_{\log n}$ contribute an additive $O(L) Opt$ to our expected completion time.
	
	Now it suffices to show that the expected completion time of $J_{\log n}$ is at most $O(\alpha L \sqrt{m} \cdot poly(\log n)) Opt$. For these jobs, we relate their starting times to the expected starting time of Opt. We can partition $J_{\log n}$ into $J_k \setminus J_{k-1}$ for all $k$, where $\lvert J_k \setminus J_{k-1} \rvert = O(L \cdot n/2^k)$, and all jobs in $J_k$ have starting time at most $\tilde{F}(J_k)$, by definition. Combined with the guarantees of the assumed Batch Free Time algorithm and \Cref{thm_batches_opt_cost}, we have:
	\begin{align*}
	    \sum_{j \in J_{\log n}} \mathbb{E} S_j &\leq L \sum_k  O(n/2^k) \cdot \mathbb{E} \tilde{F}(J_k)\\
	    &= O(\alpha L) \sum_k  n/2^k \cdot \mathbb{E} \tilde{F}^*(J_k)\\
	    &= O(\alpha L \sqrt{m} \cdot poly(\log n))(\sum_k n/2^k \cdot \mathbb{E} F^*(n - n/2^k) + Opt).
	\end{align*}
 
	 
	It remains to relate $\sum_k n/2^k \cdot \mathbb{E} F^*(n - n/2^k)$ to $Opt$ We note that $\Omega(n/2^k)$ jobs have starting times in $[F^*(n - n/2^{k-1}), F^*(n - n/2^k)]$ in $Opt$, so we can further bound:
	\[\sum\limits_k n/2^k \mathbb{E} F^{Opt}(n- n/2^k) = \Omega(Opt).\]
	Combining the two bounds completes the proof.
\end{proof}

Note that we crucially used the fact that an algorithm for Batch Free Time Minimization outputs a list schedule to bound the completion time of the jobs $J \setminus J_{\log n}$. In the remainder of this paper, we give an efficient algorithm for the latter problem, which implies the desired completion time algorithm.


==> final_approx.tex <==
\section{Final Approximation Algorithm}\label{sec_final_approx}

In this section, we prove our main result: \Cref{thm_mainber}. To do so, we prove a meta-theorem parametrized by the number of distinct size parameters, $L$.

\begin{theorem}\label{thm_mainsize}
	There exists an efficient algorithm that computes a $O(L \sqrt{m} \cdot poly(\log n))$-approximate list schedule for minimizing completion time of Bernoulli jobs.
\end{theorem}
\begin{proof}
	By \Cref{thm_batchreduce}, it suffices to show that there exists an efficient algorithm for Batch Free Time Minimization for Bernoulli jobs with $L$ sizes and $\alpha = O(1)$. This is exactly the algorithm guaranteed by \Cref{thm_warmreduce}.
\end{proof}

\Cref{thm_mainber} is a corollary of this theorem. For general Bernoulli jobs, the next lemma states that we can assume the Bernoulli size parameters are polynomially-bounded without loss of generality. The proof is a rescaling argument. Then by losing a constant-factor in our final approximation ratio, we may assume the size parameters are bounded in $[1, poly(n)]$ and round them up to the nearest power of two. This gives $L = O(\log n)$, as desired.

\begin{lem}\label{lem_bernoilli_rescale}
    Suppose there exists an algorithm that is $\alpha$-approximate for minimizing completion time of Bernoulli jobs with size parameters bounded in $[1, n^c]$. Then there exists an $O(\alpha)$-approximate algorithm for minimizing completion time of Bernoulli jobs with arbitrary size parameters.
\end{lem}
\begin{proof}\alert{can probably simplify}
    If the number of machines $m = 1$, then the lemma is trivial, because SEPT is optimal for minimizing completion time of stochastic jobs on one machine. Thus, we may assume $m \geq 2$. Let $\mathcal{A}$ be the algorithm guaranteed by the lemma.
    
    Suppose we have a collection $J$ of Bernoulli jobs of the form $X_j \sim s_j Ber (p_j)$ for arbitrary size parameters $s_j$. Let $Opt$ be a random variable denoting the completion time of the optimal scheduling policy on jobs $J$. Without loss of generality, we may assume $\sum_{j \in J} \mathbb{E} X_j = 1$ by rescaling all $s_j$'s uniformly. Note that $\sum_{j \in J} \mathbb{E} X_j \leq \mathbb{E} Opt$, so $\mathbb{E} Opt = \Omega(1)$. Our algorithm to schedule $J$ is the following:
    \begin{enumerate}
        \item List-schedule all small jobs $S = \{j \in J \mid s_j < \frac{1}{n^2}\}$ in arbitrary order.
        \item Every machine will be free by time $\frac{1}{n}$. At time $\frac{1}{n}$, we run algorithm $\mathcal{A}$ on the \emph{modified} remaining jobs $\tilde{X}_j  = X_j 1_{X_j \leq n^c}$ for all $j \in \tilde{J} = J \setminus S$ in order to schedule the \emph{actual} jobs $X_j$.
        \item If some job $X_j$ scheduled by $\mathcal{A}$ has realized size $X_j > n^c$ (i.e. $X_j \neq \tilde{X}_j$), then we stop following $\mathcal{A}$'s schedule, and instead list-schedule all remaining jobs in arbitrary order. Otherwise, we run $\mathcal{A}$'s schedule to completion.\label{step_simulate_alg}
    \end{enumerate}
    Note that every $\tilde{X}_j$ for $j \in \tilde{J}$ has size parameter in $[\frac{1}{n^2}, n^c]$, so $\{\tilde{X_j} \mid j \in \tilde{J}\}$ is a valid input for $\mathcal{A}$.
    
    It remains to bound the cost of this schedule. The completion time of all jobs in $S$ can be crudely upper-bounded by the max load after $S$ times the number of jobs, which is at most $n \cdot \frac{1}{n} = O( \mathbb{E} Opt)$. After this, we schedule $\tilde{J}$ using $\mathcal{A}$ at time $\frac{1}{n}$. Starting at time $\frac{1}{n}$ as opposed to time $0$ increases the completion time of each job by $\frac{1}{n}$. This increases the total completion time by at most $n \cdot \frac{1}{n} = O(\mathbb{E} Opt)$. Let $\tilde{\mathcal{A}}$ be the algorithm (and its cost) defined in (\ref{step_simulate_alg}) starting at time $\frac{1}{n}$. To summarize, the total completion time of our algorithm is:
    \[\mathbb{E} Alg \leq n \cdot \frac{1}{n} + n \cdot \frac{1}{n} + \mathbb{E} \tilde{\mathcal{A}} = O(\mathbb{E} Opt) + \mathbb{E} \tilde{\mathcal{A}}.\]
    To analyze $\mathbb{E} \tilde{\mathcal{A}}$, we define the event $B = \{\max_{j \in \tilde{J}} X_j > n^c\}$, and decompose the expectation:
    \[\mathbb{E} \tilde{\mathcal{A}} = \mathbb{E} \tilde{\mathcal{A}} 1_B + \mathbb{E} \tilde{\mathcal{A}} 1_{\bar{B}}.\]
    Observe that on the event $\bar{B}$, $\tilde{X}_j = X_j$ for all $j \in \tilde{J}$, so $\tilde{\mathcal{A}}$ agrees with $\mathcal{A}$. By the guarantees of $\mathcal{A}$, we have $\mathbb{E} \tilde{\mathcal{A}} 1_{\bar{B}} = O(\alpha) \mathbb{E} Opt$.
    
    It remains to bound $ \mathbb{E} \tilde{\mathcal{A}} 1_B$. On $B$, we upper bound $\tilde{\mathcal{A}}$ by the cost of an arbitrary list schedule of $\tilde{J}$. We define $S_1 = \max_{j \in \tilde{J}} X_j$ and $S_2$ to be the size of the second-largest job in $\tilde{J}$. On the event $B \cap \{S_2 \leq \frac{1}{n^2} S_1\}$, we note that no job is scheduled after the largest job with size $S_1$ on the same machine (using $m \geq 2$.) Noting all other jobs have size at most $\frac{1}{n^2} S_1$, we can upper bound $\tilde{\mathcal{A}}$ by $n \cdot \frac{1}{n} S_1 + S_1 = 2S_1 \leq 2 Opt$, so we have $\mathbb{E} \tilde{\mathcal{A}} 1_{B, S_2 \leq \frac{1}{n^2} S_1} = O(\mathbb{E} Opt)$.
    
    Finally, we bound $\mathbb{E} \tilde{\mathcal{A}} 1_{B, S_2 > \frac{1}{n^2} S_1}$. We partition $B = \cup_{k = 0}^\infty B_k$, where $B_k = \{\max_{j \in \tilde{J}} X_j \in [2^k n^c, \, 2^{k+1} n^c)\}$. On the event $B_k \cap \{S_2 > \frac{1}{n^2} S_1\}$, there are at least two jobs of size at least $2^k n^{c-2}$. Recall that $\sum_{j \in J} \mathbb{E} X_j = 1$, so in particular $\mathbb{E} X_j \leq 1$ for all $j \in \tilde{J}$. Thus by Markov's inequality, $\mathbb{P}(X_j \geq 2^k n^{c-2}) \leq 2^{-k} n^{-c+2}$ for all $j \in \tilde{J}$. By union-bounding over all pairs of jobs in $\tilde{J}$:
    \[\mathbb{P}(B_k, \, S_2 > \frac{1}{n^2} S_1) \leq \mathbb{P}(\text{$\exists$ two jobs in $\tilde{J}$ with size at least $2^k n^{c-2}$}) \leq O(n^2) (2^{-k} n^{-c+2})^2.\]
    Further, on the event $B_k \cap \{1_{B, S_2 > \frac{1}{n^2} S_1}\}$, every job has size at most $2^{k+1} n^c$, so we have $\tilde{\mathcal{A}} \leq n \cdot n 2^{k+1}n^c = 2^{k+1} n^{c+2}$. Thus, for each $k$, we have:
    \begin{align*}
        \mathbb{E} \tilde{\mathcal{A}} 1_{B_k, S_2 > \frac{1}{n^2} S_1} &\leq 2^{k+1} n^{c+2} \mathbb{P}(B_k, \, S_2 > \frac{1}{n^2} S_1)\\
        &= 2^{k+1} n^{c+2} O(n^2) (2^{-k} n^{-c+2})^2 = O(2^{-k}).
    \end{align*}
    To complete the proof, we partition $B = \cup_{k = 0}^\infty B_k$ to bound $\mathbb{E} \tilde{\mathcal{A}} 1_{B, S_2 > \frac{1}{n^2} S_1}$:
    \[\mathbb{E} \tilde{\mathcal{A}} 1_{B, S_2 > \frac{1}{n^2} S_1} = \sum_{k = 0}^\infty  \mathbb{E} \tilde{\mathcal{A}} 1_{B_k, S_2 > \frac{1}{n^2} S_1} = O(\sum_{k = 0}^\infty 2^{-k}) = O(\mathbb{E} Opt).\]
\end{proof}


==> free_time_prelim.tex <==
\section{From Completion Time to Free Times}\label{sec_free_time_prelim}

Our first observation is that to bound the completion time of a job, it suffices to bound its \emph{starting time}. For a particular schedule, the starting time of job $j$ is the time when job $j$ is started, which we denote by $S_j$. Importantly, on identical machines we have $C_j = S_j + X_j$.

To motivate our algorithm for minimizing completion time, we first simplify the objective by ``bucketing" similar starting times into groups. To this end, consider any fixed schedule. For $i = 1, \dots, n$, let $S(i)$ denote the \emph{$i$th starting time}, which is the time that the $i$th job is started. This differs from $S_j$, which is the starting time of a particular job $j$. By definition, we have:
\[\sum_j S_j = \sum_{i = 1}^n S(i).\]
Further, for any $i < i'$, there are $i' - i +1$ jobs with starting times in $[S(i), S(i')]$. Using this observation, we can partition the jobs into $\log n$ groups of sizes $\Theta(n/2^k)$ for $k = 1, \dots, \log n$ by considering the jobs with starting times in $[S(n- n/2^{k-1}), S(n - n/2^k)]$ for all such $k$. It follows:
\[\sum_{i = 1}^n S(i) = \sum_{k = 1}^{\log n} \Theta(n/2^k) S(n - n/2^k).\]

Algorithmically, it will be more convenient to work with what we call \emph{free times} rather than starting times.

\begin{definition}[Free Time]
	Consider any fixed schedule. The $i$th free time of the schedule, which we denote by $F(i)$ is the first time when $i$ jobs have been started and a machine is free.
\end{definition}

By definition of free time, we have $S(i) \leq F(i) \leq S(i + 1)$ for all $i$. Thus, it still holds that there are $\Theta(n/2^k)$ jobs with starting times in $[F(n- n/2^{k-1}), F(n - n/2^k)]$ for all $k$, so we have:
\[\sum_{i = 1}^n S(i) = \sum_{k = 1}^{\log n} \Theta(n/2^k) F(n - n/2^k).\]

We interpret this final expression as defining $\log n$ ``work checkpoints" for our algorithm. These checkpoints are the time that we have $n/2$ jobs left to start, so $F(n-n/2^1)$, $n/4$ left to start, so $F(n-n/2^2)$, and so on. Roughly, the goal of our algorithm is to ensure that at each work checkpoint, our time is comparable with the optimal schedule's time at the same checkpoint.

==> order_jobs.tex <==
\section{Batch Free Time Minimization}\label{order_jobs}

The goal of this section is to solve Batch Free Time Minimization. We re-state the problem here for convenience:

\begin{definition}[Batch Free Time Minimization, re-stated]
	Given nested sets of stochastic jobs, $J_1 \subset \dots \subset J_K$, we want to construct a \emph{list schedule} of $J_K$ subject to the constraint that we must start all jobs in $J_{k-1}$ before any job in $J_k \setminus J_{k-1}$ for all $k$. The goal is to guarantee that $\mathbb{E} \tilde{F}(J_k) \leq \alpha (\mathbb{E} \tilde{F}^*(J_1) + \cdots + \mathbb{E} \tilde{F}^*(J_k))$ for all $k$ simultaneously and some $\alpha \geq 1$, where $\tilde{F}(J_k)$ is free time of $J_k$ achieved by our algorithm, and $\tilde{F}^*(J_k)$ is analogous optimal free time (subject to the same constraint.)
\end{definition}

The two main difficulties of this problem are the randomness in the job sizes and the batch constraints (we must start one batch completely before the next.) As a warm-up, we first solve the problem for deterministic jobs and a single batch. Surprisingly, it turns out that we can reduce the general case to this simple warm-up.

\subsection{Warm Up: Free Time for Deterministic Jobs}

We define a simpler, optimization variant of Batch Free Time Minimization.

\begin{definition}[Free Time Minimization for Deterministic Jobs]
	Given a set of deterministic jobs, $J$, the goal is to list-schedule $J$ to minimize $F(J)$.
\end{definition}

While this problem seems similar to makespan minimization (given deterministic jobs, schedule them to minimize the load of the most-loaded machine), we note that an arbitrary list schedule is $\Omega(m)$-approximate for free time, while it is $O(1)$-approximate for makespan.

\begin{lem}\label{lem_freelower}
	For all $m > 1$, there exists a set of jobs $J$ and a list-schedule of $J$ whose free time is $\Omega(m)$-approximate.
\end{lem}
\begin{proof}
	Consider $m$ small jobs of size $1$ and $m-1$ big jobs of size $m$. The optimal free time schedule is to first schedule one small job on each machine, and then one big job on $m-1$ machines. Thus the optimal free time is $1$.
	
	Now consider the list-schedule of all big jobs before small jobs. Then each big job is scheduled on a separate machine, and all $m$ small jobs are scheduled on the remaining machine. This gives free time $m$.
\end{proof}

The instances from \Cref{lem_freelower} suggest that we should schedule small jobs before bigger ones so that the big jobs do not ``clog up" the machines and delay the starting times of the small jobs. This intuition turns out to be correct, which we formalize in the next theorem.

\begin{theorem}\label{thm_singlefree}
	List-scheduling deterministic jobs in increasing order of size is a $4$-approximation for free time.
\end{theorem}
\begin{proof}
	Let $J$ be the set of input jobs and $Opt$ the optimal free time. We partition $J$ into \emph{small} and \emph{big} jobs. A job is big if its size is strictly greater than $Opt$ and small otherwise.
	
	By our definition of big, Opt can schedule at most one big job per machine. Further, there are strictly less than $m$ big jobs. Otherwise Opt would need to schedule at least one big job per machine, which contradicts the optimal free time.
	
	On the other hand, our algorithm starts all small jobs before all big jobs. We claim that $F(J)$ is at most the makespan of our algorithm after only scheduling the small jobs, which we denote by $M(S)$. To see this, consider the time right before we start the first big job. All machines have loads within $[M(S) - Opt, M(S)]$ (the lower bound follows by noting that we list-scheduled only jobs of size at most $Opt$ up until this point.) Thus, we schedule the $m-1$ remaining big jobs each on separate machines. All of the big jobs are started by time $M(S)$, and the machine that schedules no big job is free by $M(S)$ as well. It follows, $F(J) \leq M(S)$.
	
	Now, because every list-schedule is $2$-approximate for makespan, we have $M(S) \leq 2 M^{Opt} (S)$, where $M^{Opt}(S)$ is the makespan of the small jobs under Opt (i.e. when Opt finishes its final small job.) To complete the proof, we relate $M^{Opt}(S)$ with $Opt$. It suffices to show $M^{Opt}(S) \leq 2 Opt$. To see this, consider time $Opt$ in the optimal schedule. At this time, all machines are either free or working on their final job. In particular, any machine working on a small job completes by time $Opt + Opt$.
\end{proof}

\subsection{Extending to Batches of Bernoulli Jobs}

With our warm-up in hand, we now discuss how to reduce Batch Free Time Minimization with Bernoulli jobs to Free Time Minimization with deterministic jobs. The main goal of this section is to prove the following theorem.

\begin{theorem}\label{thm_warmreduce}
	List-scheduling jobs in each batch in increasing order of their size parameters solves Batch Free Time Minimization for Bernoulli jobs with $\alpha = 5$.
\end{theorem}

We begin with the transition from deterministic jobs to Bernoulli jobs. Even if we had only a single batch of Bernoullis, we cannot hope to schedule the jobs in increasing order of their realized size. However, what we can do it schedule them in increasing order of their size parameters. It turns out, this allows us to simulate the list-schedule of \Cref{thm_singlefree} conditioned on the realizations of the job sizes.


\begin{lem}\label{lem_bernoullisingle}
	List-scheduling Bernoulli jobs in increasing order of their size parameters is a $4$-approximation for free time on a per-realization basis.
\end{lem}
\begin{proof}
	Consider any realization of job sizes. Let $J$ denote the set of \emph{deterministic} jobs obtained by conditioning the input Bernoulli jobs on this realization. Thus, we wish to show that $F(J) \leq 4 F^*(J)$. Let $J' \subset J$ be the set of jobs whose realized size is non-zero (i.e. their realized size is equal to their size parameter.) By definition of our algorithm, for jobs in $J'$, we schedule them in increasing order of their realized size.
	
	On the other hand, the jobs with zero realized size do not effect the free time because our algorithm is a list schedule. Thus, applying \Cref{thm_singlefree} gives:
	\[F(J) = F(J') \leq 4 F^*(J') \leq 4 F^*(J).\]
\end{proof}

To handle multiple batches of jobs, we introduce the concept of \emph{initial loads}. Consider scheduling batch $J_2$ after $J_1$. We view scheduling $J_2$ as a separate instance of free time minimization, where each machine starts with some initial load (determined by our schedule of $J_1$.) The main idea is to show that for all $k$, when we schedule batch $J_k$ the initial load of our algorithm is comparable to the initial load of the optimal schedule. Then by appealing to some basic monotonicity properties of list-schedules, we show roughly that the initial loads do not affect the result of \Cref{thm_singlefree}.

\begin{proof}[Proof of \Cref{thm_warmreduce}]
	Consider any realization of the job sizes, say $r$. It suffices to show that our algorithm achieves $\tilde{F}_r(J_k) \leq 5 (\tilde{F}^*_r(J_1) + \cdots + \tilde{F}^*_r(J_k))$ for all $k$, where the subscript $r$ denotes that we condition on realization $r$. We will prove this by induction on $k=1, \dots, K$.
	
	In the base case $k=1$, \Cref{lem_bernoullisingle} immediately implies $\tilde{F}_r(J_1) \leq 4 \tilde{F}^*_r(J_1)$, as required.
	
	Now for the inductive case $k >1$, we assume inductively that $\tilde{F}_r(J_{k-1}) \leq 5 (\tilde{F}^*_r(J_1) + \cdots + \tilde{F}^*_r(J_{k-1}))$. For this inductive step, we say a job is \emph{big} if its realized size is strictly greater than $\tilde{F}^*_r(J_k)$ and \emph{small} otherwise. Now consider the optimal schedule of $J_k$ achieving free time $\tilde{F}^*_r(J_k)$.
	
	We claim that there are strictly less than $m$ big jobs in $J_{k-1}$. Suppose not. By definition of big, Opt can schedule at most one big job per machine to achieve free time $\tilde{F}^*_r(J_k)$. However, there are at least $m$ big jobs by assumption, so Opt must schedule at least one per machine. This contradicts the optimal free time.
	
	Now we relate the initial loads that our algorithm and Opt experience when scheduling $J_k \setminus J_{k-1}$ after $J_{k-1}$. We define $m' = m - \#\{\text{big jobs in $J_{k-1}$}\}$. By the previous claim, $m' > 0$. Now consider Opt scheduling $J_k \setminus J_{k-1}$ after $J_{k-1}$. Any machine that already started a big job from $J_{k-1}$ is not used to schedule any job in $J_k \setminus J_{k-1}$. Further, Opt scheduled each big job on a separate machine, so the optimal schedule schedules $J_k \setminus J_{k-1}$ on $m'$ machines each with initial load at least $\tilde{F}^*_r(J_{k-1})$.
	
	On the other hand, for our algorithm, consider time $\tilde{F}_r(J_{k-1})$. At this time, all jobs in $J_{k-1}$ are finished or currently in progress. In particular, at least $m'$ machines are free or scheduling small jobs. These machines can start $J_k \setminus J_{k-1}$ by time $\tilde{F}_r(J_{k-1}) + \tilde{F}^*_r(J_k)$. Thus, our algorithm schedules $J_k \setminus J_{k-1}$ on at least $m'$ machines each with initial load at most $\tilde{F}_r(J_{k-1}) + \tilde{F}^*_r(J_k)$.
	
	To complete the proof, we need the following monotonicity property of list schedules. 
	
	\begin{lem}\label{lem_listprop}
		Consider a set of deterministic jobs and a fixed list schedule of those jobs. Then increasing the initial load or decreasing the number of machines weakly increase the free time of the schedule.
	\end{lem}
	\begin{proof}
		Let $J$ be the set of jobs. Consider initial load vectors $\ell, \ell' \in \mathbb{R}^m$, where the $i$th entry of each vector denotes the initial load on machine $i$. Now suppose $\ell \leq \ell'$, entry-wise. It suffices to show that $F(J,\ell) \leq F(J,\ell')$, where $F(J,\ell)$ is the free time achieved by our list-schedule with initial load $\ell$. This suffices, because we can decrease the number of machines by making the initial loads of some machines arbitrarily large so that they will never be used.
		
		We prove $F(J,\ell) \leq F(J,\ell')$ by induction on the number of jobs, $\lvert J \rvert$.
		In the base case, $\lvert J \rvert = 0$, so the claim is trivial because $\ell \leq \ell'$.
		For $\lvert J \rvert > 0$, let $j$ be the first job in the list, which is scheduled, without loss of generality, on the first machine for both initial loads $\ell$ and $\ell'$. Then:
		\[F(J,\ell) = F(J \setminus \{j\}, \ell + s_j e_1) \leq F(J \setminus \{j\}, \ell' + s_j e_1) = F(J,\ell'),\]
		where we assumed inductively that $F(J \setminus \{j\}, \ell + s_j e_1) \leq F(J \setminus \{j\}, \ell' + s_j e_1)$, and $e_1$ is the first standard basis vector.
	\end{proof}

	Using the lemma, we can bound $\tilde{F}_r(J_k)$ with respect to $F_r(J_k \setminus J_{k-1})$ and our algorithm's initial load. Recall that our algorithm schedules $J_k \setminus J_{k-1}$ on at least $m'$ machines with initial loads at most $\tilde{F}_r(J_{k-1}) + \tilde{F}^*_r(J_k)$. However, decreasing the number of machines to $m'$ and increasing their initial loads to $\tilde{F}_r(J_{k-1}) + \tilde{F}^*_r(J_k)$ can only increase the free time by the lemma. Thus:
	\[\tilde{F}_r(J_k) \leq (\tilde{F}_r(J_{k-1}) + \tilde{F}^*_r(J_k)) + F_r(J_k \setminus J_{k-1}, m'),\]
	where $F_r(J_k \setminus J_{k-1}, m')$ is defined to be the free time with $m'$ machines (as opposed to the initial $m$.)
	Now observe that our algorithm schedules $J_k \setminus J_{k-1}$ in increasing order of size parameter, so \Cref{lem_bernoullisingle} gives $F_r(J_k \setminus J_{k-1}, m') \leq 4 F^*_r(J_k \setminus J_{k-1}, m')$. Also, recall that we assumed inductively that $\tilde{F}_r(J_{k-1}) \leq 5 (\tilde{F}^*_r(J_1) + \cdots + \tilde{F}^*_r(J_{k-1}))$. Combining these inequalities gives the following upper bound on our algorithm's free time:
	\[\tilde{F}_r(J_k) \leq 5(\tilde{F}^*_r(J_1) + \cdots + \tilde{F}^*_r(J_{k-1})) + \tilde{F}^*_r(J_k)) + 4 F^*_r(J_k \setminus J_{k-1}, m').\]
	
	We lower bound $F^*_r(J_k)$ similarly with respect to $F^*_r(J_k \setminus J_{k-1})$ and Opt's initial load. We recall that Opt schedules $J_k \setminus J_{k-1}$ on at most $m'$ machines with initial loads at least $\tilde{F}^*_r(J_{k-1})$. Then we can lower bound:
	\[F^*_r(J_k) \geq \tilde{F}^*_r(J_{k-1}) + F_r^*(J_k \setminus J_{k-1}, m').\]
	Combining the upper and lower bounds for our algorithm and Opt, respectively, gives:
	\[\tilde{F}_r(J_k) \leq 5(\tilde{F}^*_r(J_1) + \cdots + \tilde{F}^*_r(J_{k-1})) + 5 \tilde{F}^*_r(J_k) - 4 \tilde{F}^*_r(J_{k-1}) \leq 5(\tilde{F}^*_r(J_1) + \cdots + \tilde{F}^*_r(J_k)).\]
\end{proof}


==> prove_batches_opt_cost.tex <==
\section{\choosealg Analysis: Proof of \Cref{thm_batches_opt_cost}}\label{sec_prove_batches_opt_cost}

The goal of this section is to prove \Cref{thm_batches_opt_cost}. Let $J_1, \dots, J_{\log n}$ be the sets of jobs output by \choosealg. We recall that $J_k^*$ is the random set of the first $n-n/2^k$ jobs scheduled by the optimal completion time policy, $Opt$.

We first introduce some notations. For all $k$, we call $I_k = J_k \setminus J_{k-1}$ the $k$th \emph{batch} of jobs. Recall that the $J_k$'s are nested, so the batch constraint says we schedule in order $I_1, \dots, I_{\log n}$. We define $I_k^* = J_k^* \setminus J_{k-1}^*$ analogously. For any set of jobs, $J'$ and $\tau \geq 0$, we define $J'(=\tau)$ to be the random subset consisting of all jobs in $J'$ with \emph{realized} size exactly $\tau$. We define $J'(>\tau)$ and $J'(\leq \tau)$ analogously. Further, for a set of jobs $J'$, we let $Vol(J') = \sum_{j \in J'} X_j$ be the volume of $J'$. Finally, we say job $j$ is $\tau$-big for $\tau \geq 0$ if $X_j > \tau$. Otherwise $j$ is $\tau$-small.

To prove \Cref{thm_batches_opt_cost}, we give an existential schedule \alert{should clarify in theorem statement that schedule can be clairvoyant} satisfying the batch constraint that is comparable to $Opt$. The particular schedule we consider is to list-schedule each $I_k$ in increasing order of \emph{realized} size. Thus, to prove \Cref{thm_batches_opt_cost}, it suffices to show:
\[\sum_{k =1}^{\log n} n/2^k \cdot \mathbb{E} \tilde{F}(J_k) = O(\sqrt{m} \cdot poly(\log n)) (\sum_{k =1}^{\log n} n/2^k \cdot \mathbb{E} F^*(n-n/2^k) + \sum_j \mathbb{E} C_j^*),\]
where $\tilde{F}(J_k)$ is the free time of $J_k$ achieved by the schedule that list-schedules each $I_k$ in increasing order of realized size.

As in the analysis for Batch Free Time Minimization, the key concept is to differentiate between small and big jobs. To this end, for all $k$ we define $\tau_k = 2 \max(\mathbb{E} F^*(n - n/2^k), F^*(n - n/2^k))$. Morally, one should imagine that $\tau_k$ is $F^*(n - n/2^k)$, but there is an edge case where $F^*(n - n/2^k) < \mathbb{E} F^*(n - n/2^k)$ and a multiplicative factor for concentration. When bounding $\tilde{F}(J_k)$, we will take $\tau_k$ to be our threshold between small- and big jobs. This threshold has the following crucial property:
    
\begin{prop}\label{prop_big_threshold}
    For all $k$, the following holds per-realization: $\lvert J_k(> \tau_k) \rvert \leq \lvert J_k^*(> \tau_k) \rvert < m$.
\end{prop}
\begin{proof}
    The first inequality follows from \Cref{lem_batch_prefix}, because $J_k(> \tau_k) \subset J_k^*(> \tau)$ per-realization. For the second inequality, note that $\tau_k \geq F^*(n - n/2^k)$, so by definition of free time, $Opt$ schedules strictly less than $m$ jobs bigger than $\tau_k$ to achieve $F^*(n-n/2^k)$. 
\end{proof}

Using this threshold, we re-write $\tilde{F}(J_k)$ by averaging the volume of small jobs over the machines with no big job:

\begin{prop}\label{prop_k_free_vol}
    For all $k$, the following holds per-realization:
    \[\tilde{F}(J_k) \leq \tilde{F}(J_{k-1}) + \frac{Vol(I_k(\leq \tau_k))}{m- \lvert J_{k-1}(> \tau_k) \rvert} + 2 \tau_k.\]
\end{prop}
\begin{proof}
    First, we note by \Cref{prop_big_threshold} that the denominator $m - \lvert J_{k-1}(> \tau_k) \rvert \geq 1$. Then consider time $\tilde{F}(J_{k-1})$. There are at least $m - \lvert J_{k-1}(> \tau_k) \rvert$ machines that have not scheduled a $\tau_k$-big job in $J_{k-1}$. At this time, each machine is either free or working on its final job in $J_{k-1}$. In particular, each machine that has not scheduled a $\tau_k$-big job in $J_{k-1}$ is free to start working on $I_k$ by time $\tilde{F}(J_{k-1}) + \tau_k$, and there are at least $m - \lvert J_{k-1}(> \tau_k) \rvert$ such machines.
    
    By \Cref{lem_listprop}, we can upper-bound $\tilde{F}(J_k)$ by list-scheduling $I_k$ with initial load $\tilde{F}(J_{k-1}) + \tau_k$ on $m - \lvert J_{k-1}(> \tau_k) \rvert$ machines. Recall we list-schedule $I_k$ in increasing order of realized size, and there are strictly less than $m$ $\tau_k$-big jobs in $J_k$, so there exists some machine that schedules only $\tau_k$-small jobs in $I_k$. This machine is free by time $\tilde{F}(J_k) \leq \tilde{F}(J_{k-1}) + \tau_k + \frac{Vol(I_k(\leq \tau_k))}{m- \lvert J_{k-1}(> \tau_k) \rvert} + \tau_k$.
\end{proof}

Using~\Cref{prop_k_free_vol} and the exponentially decreasing weights, we have:
\[\sum_{k =1}^{\log n} n/2^k \cdot \tilde{F}(J_k) = O (\sum_k n/2^k \cdot \frac{Vol(I_k(\leq \tau_k))}{m- \lvert J_{k-1}(> \tau_k) \rvert} + \sum_k n/2^k \cdot \tau_k).\]
By definition of $\tau_k$, the second sum is $O(\sum_k n/2^k \cdot \mathbb{E} F^*(n-n/2^k))$ in expectation. It remains to bound the first sum. The main challenge in bounding the first sum is that even though $J_k \subset J_k^*$ for all $k$, it is not true that $I_k \subset I_{k^*}$. This means that while we are averaging $Vol(I_k(\leq \tau_k))$ over $m - \lvert J_{k-1}(> \tau_k) \rvert$ machines (which is at least as many machines as $Opt$ has for batch $k$), it can be the case that $Opt$ actually did jobs in $I_k$ in much earlier batches. Thus, $Opt$ could potentially average the same volume over many more machines, as fewer machines were clogged by $\tau_k$-big jobs in the past. To remedy this, we control the rate that \choosealg clogs machines so that even though we do some small volume later on fewer machines than $Opt$, this is offset by the number of jobs $Opt$ delays by doing those jobs earlier.

\subsection{Bounding the clogged machines}

In this section, we are interested in controlling the quantity $m - \lvert J_{k-1}(> \tau_k) \rvert$, which is the number of machines we have left to schedule $I_k$. Note that there are two sources of randomness: the realizations of jobs in $J_{k-1}$ and the threshold $\tau_k$.

We first consider a fixed threshold, say $\tau$ and focus on $J_{k-1}(> \tau)$. We first use the properties of \choosealg to bound $\mathbb{E} \lvert J_{k-1}(> \tau) \rvert$:

\begin{prop}\label{prop_batch_decrease}
    For all sizes $s$ and batches $k$, we have $\mathbb{E} \lvert I_k(>s) \rvert \geq \frac{1}{2} \mathbb{E} \lvert I_{k-1}(>s)\rvert$.
\end{prop}
\begin{proof}
    By summing over the relevant sizes, it suffices to prove $\mathbb{E} \lvert I_k(=s) \rvert \geq \frac{1}{2} \mathbb{E} \lvert I_{k-1}(=s)\rvert$. We may assume $\mathbb{E} \lvert I_{k-1}(=s)\rvert > 0$ or else the proposition is trivial. 
    
    Then when \choosealg constructs $J_{k-1}$, it includes at least one job with size parameter $s$. It follows, there exist $n/2^{k-1}$ remaining jobs in $J \setminus J_{k-1}$ with size parameter $s$. When constructing $J_k$, \choosealg will include $n/2^k$ of these remaining jobs. In conclusion, $I_{k-1}$ has at most $n/2^{k-1}$ jobs with size parameter $s$, while $I_k$ has at least $n/2^k$. The result follows because \choosealg includes jobs in increasing order of $p_j$.
\end{proof}

\Cref{prop_batch_decrease} allows us to relate the expected number of machines left (with respect to fixed threshold $\tau$) at batch $k$ with the number of machines left at $k' \leq k$:

\begin{lem}\label{lem_machine_remain}
    For all sizes $s$ and batches $k' \leq k$, we have $m' - \mathbb{E}\lvert J_{k-1}(> s) \rvert \geq 2^{-(k-k' + 1)} \cdot (m' - \mathbb{E}\lvert J_{k'-1}(> s)\rvert)$, where $m' \geq \mathbb{E} \lvert J_k(>s) \rvert$.
\end{lem}
\begin{proof}
    We may assume $\mathbb{E} \lvert I_k(>s) \rvert > 0$ or else the lemma is trivial, because by definition of \choosealg, if $\mathbb{E} \lvert I_k(>s) \rvert = 0$, then $\mathbb{E} \lvert J_{k-1}(>s)\rvert = 0$ and $\mathbb{E} \lvert J_{k'-1}(>s)\rvert = 0$.
    
    In particular, we may assume $m' - \mathbb{E} \lvert J_{k-1}(>s) \rvert \geq \mathbb{E} \lvert I_{k}(>s) \rvert > 0$. Then we compute:
    \[\frac{m' - \mathbb{E} \lvert J_{k' -1}(>s) \rvert}{m' - \mathbb{E} \lvert J_{k -1}(>s) \rvert} = 1 + \frac{\mathbb{E} \lvert I_{k'}(>s) \rvert + \dots + \mathbb{E} \lvert I_{k-1}(>s) \rvert}{m' - \mathbb{E} \lvert J_{k -1}(>s) \rvert} \leq 1 + \frac{\mathbb{E} \lvert I_{k'}(>s) \rvert + \dots + \mathbb{E} \lvert I_{k-1}(>s) \rvert}{\mathbb{E}\lvert I_{k}(>s) \rvert}.\]
    Repeatedly applying \Cref{prop_batch_decrease} to the numerator gives:
    \[1 + \frac{\mathbb{E} \lvert I_{k'}(>s) \rvert + \dots + \mathbb{E} \lvert I_{k-1}(>s) \rvert}{\mathbb{E}\lvert I_{k}(>s) \rvert} \leq 1 + (2^{k-k'} + \dots + 2^1) \leq 2^{k-k' + 1}.\]
\end{proof}

To see the utility of \Cref{lem_machine_remain}, suppose $\mathbb{E}
\lvert J_k (>s) \rvert = m$. Then roughly the lemma says that in expectation, we lose at most half of our remaining machines between each batch. To take advantage of this, note that $\lvert J_{k-1}(>\tau)\rvert$ is the sum of independent $\{0,1\}$-random variables, so it is concentrated about its expectation by a standard Chernoff bound.

    \begin{prop}[Chernoff bound]\label{prop_chernoff}
        Let $X = X_1 + \dots X_n$ be a sum of independent, $\{0,1\}$-valued random variables and $\mu = \mathbb{E} X$. Then we have:
        \begin{itemize}
            \item $\mathbb{P}(X \leq (1 - \delta) \mu) \leq \exp{(-\frac{\delta^2 \mu}{2})}$ for all $0 \leq \delta \leq 1$.
            \item $\mathbb{P}(X \geq (1 + \delta) \mu) \leq \exp{(-\frac{\delta^2 \mu}{2 + \delta})}$ for all $0 \leq \delta$.
        \end{itemize}
    \end{prop}

First, we bound the expectation of $\lvert J_k(> \tau) \rvert$:

\begin{lem}\label{lem_big_job_small_expectation} \alert{not sure cleanest way to write}
    Let $m = \Omega(1)$ be sufficiently large. Then there exists a constant $c \geq 0$ such that for all batches $k$ and thresholds $\tau > 2 \mathbb{E} F^*(n-n/2^k)$, we have $\mathbb{E} \lvert J_k(> \tau) \rvert \leq m + c \sqrt{m}$.
\end{lem}
\begin{proof}
    Fix $c \geq 0$ which we will choose sufficiently large later. Then assume for contradiction that there exists a batch $k$ and threshold $\tau > 2 \mathbb{E} F^*(n-n/2^k)$ such that $\mathbb{E} \lvert J_k(> \tau) \rvert > m + c \sqrt{m}$.
    
    To reach a contradiction, it suffices to show that $\mathbb{P}(\lvert J_k(> \tau) \rvert \leq m) < \frac{1}{2}$. This is because on the complement event $\lvert J_k(> \tau) \rvert > m$ (which happens with probability strictly larger than $\frac{1}{2}$), we also have $\lvert J^*_k(> \tau) \rvert > m$ by \Cref{lem_batch_prefix}. This implies $F^*(n - n/2^k) > \tau \geq 2 \mathbb{E} F^*(n-n/2^k)$. This would contradict the definition of $\mathbb{E} F^*(n-n/2^k)$.
    
    For convenience, let $\mu = \mathbb{E} \lvert J_k (> \tau) \rvert$. By Chernoff, we have:
    \[\mathbb{P}(\lvert J_k(> \tau) \rvert \leq m) = \mathbb{P}(\lvert J_k(> \tau) \rvert \leq \mu(1 - \frac{\mu - m}{\mu})) \leq \exp{(-\frac{(\mu - m)^2}{2\mu})}.\]
    There are two cases to consider. Recall that by assumption, we have $\mu > m + c \sqrt{m}$. If $\mu \geq 2m$, then $\mathbb{P}(\lvert J_k(> \tau) \rvert \leq m) \leq \exp{(- \frac{\mu}{8})} \leq \exp{(- \frac{m}{4})} < \frac{1}{2}$ for $m = \Omega(1)$ sufficiently large. Otherwise, $m + c \sqrt{m} < \mu < 2m$. Then $\mathbb{P}(\lvert J_k(> \tau) \rvert \leq m) \leq \exp{(- \frac{c^2 m}{2m})} < \frac{1}{2}$ for $c = O(1)$ sufficiently large.
\end{proof}

Now, because $\mathbb{E} \lvert J_k(> \tau) \rvert = O(m)$, we can bound the deviation of $\lvert J_k(> \tau) \rvert$ by $\tilde{O}(\sqrt{m})$:

\begin{lem}\label{lem_big_job_chernoff}\alert{not sure cleanest way to write this}
    Let $\Delta = O(\sqrt{m} \log n)$ and $m = \Omega(1)$ be sufficiently large. Then with probability at least $1 - \frac{1}{poly(n)}$, for every batch $k$ and threshold $\tau > 2 \mathbb{E} F^*(n-n/2^k)$, we have:
    \begin{equation}\label{event_delta_big}
        \lvert J_k(> \tau) \rvert \stackrel{\pm \Delta}{\approx} \mathbb{E} \lvert J_k(> \tau) \rvert
    \end{equation}\alert{define notation?}
\end{lem}
\begin{proof}
    Note that there are $O(\log n)$ choices for $k$ and $L \leq n$ relevant choices for $\tau$. Thus, by a standard union bound argument it suffices to show that for fixed $k$ and $\tau > 2 \mathbb{E} F^*(n-n/2^k)$, we have:
    \[\mathbb{P}(\lvert \lvert J_k(> \tau) \rvert - \mathbb{E} \lvert J_k(> \tau) \rvert \rvert > \Delta) = \frac{1}{poly(n)}.\]
    
    Now we may assume $m$ is large enough so that $\mathbb{E} \lvert J_k(> \tau) \rvert \leq m + c \sqrt{m} \leq (c+1)m$ for sufficiently large constant $c \geq 0$ (guaranteed by \Cref{lem_big_job_small_expectation}.) Then we can bound the deviation of $\lvert J_k(> \tau) \rvert$ again with a Chernoff bound. Let $\mu = \mathbb{E} \lvert J_k(> \tau) \rvert$. We take $\Delta = O(\sqrt{\mu} \log n) = O(\sqrt{m} \log n)$.
    
    There are two cases to consider. If $\mu < \Delta$, then the lower tail is trivial:
    \[\mathbb{P}(\lvert J_k(> \tau) \rvert \leq \mu - \Delta) \leq \mathbb{P}(\lvert J_k(> \tau) \rvert < 0) = 0.\]
    For the upper tail we use Chernoff:
    \[\mathbb{P}(\lvert J_k(> \tau) \rvert \geq \mu + \Delta) = \mathbb{P}(\lvert J_k(> \tau) \rvert \geq (1 + \frac{\Delta}{\mu})\mu) \leq \exp{(- \frac{\Delta^2}{2\mu + \Delta})} \leq \exp{(- \frac{\Delta^2}{3\Delta})}  = \frac{1}{poly(n)}.\]
    Otherwise, $\mu \geq \Delta$, so in particular $\frac{\Delta}{\mu} \leq 1$. Then we use Chernoff for both the lower- and upper tails:
    \[\mathbb{P}(\lvert J_k(> \tau) \rvert \leq \mu + \Delta) = \mathbb{P}(\lvert J_k(> \tau) \rvert \leq (1 + \frac{\Delta}{\mu})\mu) \leq \exp{(- \frac{\Delta^2}{2\mu})} = \frac{1}{poly(n)}.\]
    \[\mathbb{P}(\lvert J_k(> \tau) \rvert \geq \mu + \Delta) = \mathbb{P}(\lvert J_k(> \tau) \rvert \geq (1 + \frac{\Delta}{\mu})\mu) \leq \exp{(- \frac{\Delta^2}{2\mu + \Delta})} \leq \exp{(- \frac{\Delta^2}{3\mu})}  = \frac{1}{poly(n)}.\]
    
\end{proof}

Combining \Cref{lem_machine_remain} and \Cref{lem_big_job_chernoff}, we can show the number of remaining machines is concentrated as well. This is the main result of this section. Recall that we defined $\tau_k = 2 \max(\mathbb{E} F^*(n - n/2^k), F^*(n - n/2^k))$, so in particular $\tau_k \geq 2 \mathbb{E} F^*(n - n/2^k)$.

\begin{lem}\label{lem_remaining_mach_concentration}
    Suppose Event (\ref{event_delta_big}) holds. Then for all pairs of batches $k' \leq k$, we have $m - \lvert J_{k-1}( > \tau_k) \rvert \geq (3\Delta)^{-1} 2^{-(k-k'+1)} (m - \lvert J_{k' -1}(> \tau_k) \rvert)$, where $\Delta = O(\sqrt{m} \log n)$.
\end{lem}
\begin{proof}\alert{to check algebra}
    Consider fixed batches $k' \leq k$, and let $\mu_k = \mathbb{E} \lvert J_k(> \tau_k) \rvert$ and $\mu_{k'} = \mathbb{E} \lvert J_k'(> \tau_k) \rvert$. Note that $\tau_k \geq 2 \mathbb{E} F^*(n - n/2^k) \geq 2 \mathbb{E} F^*(n - n/2^{k'})$, so Event (\ref{event_delta_big}) gives $\lvert J_k(> \tau_k) \rvert \stackrel{\pm \Delta}{\approx} \mu_k$ and $\lvert J_{k'}(> \tau_k) \rvert \stackrel{\pm \Delta}{\approx} \mu_{k'}$. Further, we may choose $\Delta = O(\sqrt{m} \log n)$ large enough so that $\mu_k \leq m + \Delta$. Using these approximations with \Cref{lem_machine_remain} gives:
    \begin{align*}
        m - \lvert J_k(> \tau_k) \rvert &= m + \Delta - \lvert J_k(> \tau_k) \rvert - \Delta\\
        &\geq m + \Delta - \mu_k - 2\Delta\\
        &\geq 2^{-(k-k'+1)}(m + \Delta - \mu_{k'}) - 2\Delta\\
        &\geq 2^{-(k-k'+1)}(m + \lvert J_k(> \tau_k) \rvert) - 2\Delta.
    \end{align*}
    Finally, by \Cref{prop_big_threshold}, $m - \lvert J_k(> \tau_k) \rvert \geq 1$, so rearranging gives:
    \[3\Delta(m - \lvert J_k(> \tau_k)\rvert) \geq m - \lvert J_k(> \tau_k) \rvert + 2\Delta \geq 2^{-(k-k'+1)}(m + \lvert J_k(> \tau_k) \rvert).\]
\end{proof}

To summarize, we showed that up to a multiplicative $\tilde{O}(\sqrt{m})$-factor, the number of machines remaining with respect to threshold $\tau_k$ at worst halves in each batch up to $k$.

\subsection{Bounding small-in-the-past jobs}\label{sec_small_past}

Recall that our goal is to bound $\sum_k n/2^k \cdot \frac{Vol(I_k(\leq \tau_k))}{m - \lvert J_{k-1}(> \tau_k) \rvert}$. To this end, consider fixed $k$. Because $I_k \subset J_k^* = \cup_{k' \leq k} I_k^*$ (by \Cref{lem_batch_prefix}), we can write:
\[\frac{Vol(I_k(\leq \tau_k))}{m - \lvert J_{k-1}(> \tau_k) \rvert} = \sum_{k' \leq k} \frac{Vol(I_k \cap I_{k'}^*(\leq \tau_{k'}))}{m - \lvert J_{k-1}(> \tau_k) \rvert} + \sum_{k' \leq k} \frac{Vol(I_k \cap I_{k'}^*(> \tau_{k'}, \leq \tau_k))}{m - \lvert J_{k-1}(> \tau_k) \rvert}.\]
Thus, we split $I_k$ depending on which batch $Opt$ decided to schedule that job in. Further, we split $I_k \cap I_{k'}^*$ (i.e. the jobs our algorithm does in batch $k$ that $Opt$ did in the past batch $k' \leq k$) into the jobs that are 'small-in-the-past' (size at most $\tau_{k'}$) and 'big-in-the-past' (size greater than $\tau_{k'}$ and at most $\tau_k$.)

The goal of this section is to bound the small-in-the-past jobs. This formalizes the idea that the rate at which we lose machines, guaranteed by \Cref{lem_remaining_mach_concentration}, is offset by the number of jobs $Opt$ is delaying, captured by the exponentially decreasing weights $n/2^k$. \alert{this is an important intuition, so should probably explain more} In particular, we show the following.

\begin{lem}\label{lem_small_past}
    Suppose Event (\ref{event_delta_big}) holds. Then we have:
    \[\sum_k n/2^k \cdot \sum_{k' \leq k} \frac{Vol(I_k \cap I_{k'}^*(\leq \tau_{k'}))}{m - \lvert J_{k-1}(> \tau_k) \rvert} = O(\Delta \log n \cdot \sum_k n/2^k \cdot \tau_k),\]
    where $\Delta = O(\sqrt{m} \log n)$.
\end{lem}
\begin{proof}
    Because there are $\log n$ batches, it suffices to show for fixed $k$ and $k' \leq k$ that we have $\frac{Vol(I_k \cap I_{k'}^*(\leq \tau_{k'}))}{m - \lvert J_{k-1}(> \tau_k) \rvert} = O(\Delta \cdot 2^{k-k'} \tau_{k'})$. Summing over all $k$ and $k' \leq k$ would give the desired result.
    
    We upper bound the numerator using $I_k \cap I_{k'}^* \subset I_{k'}^*$ and apply \Cref{lem_remaining_mach_concentration} to the denominator. This gives:
    \[\frac{Vol(I_k \cap I_{k'}^*(\leq \tau_{k'}))}{m - \lvert J_{k-1}(> \tau_k) \rvert} = O(\Delta \cdot 2^{k - k'} \frac{Vol(I_{k'}^*(\leq \tau_{k'}))}{m - \lvert J_{k'-1}(> \tau_k) \rvert}) = O(\Delta \cdot 2^{k - k'} \frac{Vol(I_{k'}^*(\leq \tau_{k'}))}{m - \lvert J_{k'-1}^*(> \tau_{k'}) \rvert}).\]
    In the final step, we used $J_{k' - 1} \subset J_{k' -1}^*$ (by \Cref{lem_batch_prefix}) and $\tau_k \geq \tau_{k'}$.
    
    Finally, we show $\frac{Vol(I_{k'}^*(\leq \tau_{k'}))}{m - \lvert J_{k'-1}^*(> \tau_{k'}) \rvert} = O(\tau_{k'})$. Recall that $\tau_{k'} > F^*(n-n/2^{k'})$, so $Opt$ schedules at most one $\tau_{k'}$-big job per machine in $J_{k'}^*$. In particular, $Opt$ schedules $I_{k'}^*(\leq \tau_{k'})$ only on the $m - \lvert J_{k' - 1}^*(> \tau_{k'}) \rvert$-machines that have not yet scheduled a $\tau_{k'}$-big job yet. By averaging, after scheduling $I_{k'}^*(\leq \tau_{k'})$, every machine in $Opt$ has load at least $\frac{Vol(I_{k'}^*(\leq \tau_{k'}))}{m - \lvert J_{k'-1}^*(> \tau_{k'}) \rvert} - \tau_{k'}$. This implies $F^*(n-n/2^{k'}) \geq \frac{Vol(I_{k'}^*(\leq \tau_{k'}))}{m - \lvert J_{k'-1}^*(> \tau_{k'}) \rvert} - \tau_{k'}$. Rearranging and using $\tau_{k'} > F^*(n-n/2^{k'})$ give the desired result.
\end{proof}

\subsection{Bounding big-in-the-past jobs}

The goal of this section is to bound the big-in-the-past jobs, that is:
\[\sum_k n/2^k \cdot \sum_{k' \leq k} \frac{Vol(I_k \cap I_{k'}^*(> \tau_{k'}, \leq \tau_k))}{m - \lvert J_{k-1}(> \tau_k) \rvert}.\]
For convenience, we define $I_{kk'} = I_k \cap I_{k'}^*(> \tau_{k'}, \leq \tau_k)$. Note that we cannot apply volume arguments as in \Cref{sec_small_past}, because the big-in-the-past jobs are $\tau_{k'}$-big. Instead, we will use the fact that $Opt$ schedules at most one $I_{kk'}$-job per machine.

There are two types of jobs in $j \in I_{kk'}$: We say $j$ is \emph{blocked} if $Opt$ later schedules a $\tau_k$-big job in $J_{k-1}$ on the same machine as $j$ (recall that $J_{k-1} \subset J_{k-1}^*$ by \Cref{lem_batch_prefix}.) Otherwise, $j$ is \emph{unblocked}. Further, a machine is blocked/unblocked if the $I_{kk'}$-job scheduled on that machine is blocked/unblocked. Thus we can partition $I_{kk'} = B_{kk'} \cup U_{kk'}$ into blocked and unblocked jobs, respectively.

By splitting the volume of jobs into unblocked and blocked, we can rewrite:
\[\sum_k n/2^k \cdot \sum_{k' \leq k} \frac{Vol(I_k \cap I_{k'}^*(> \tau_{k'}, \leq \tau_k))}{m - \lvert J_{k-1}(> \tau_k) \rvert}  = \sum_k n/2^k \cdot \sum_{k' \leq k} \frac{Vol(U_{kk'})}{m - \lvert J_{k-1}(> \tau_k) \rvert} + \sum_k n/2^k \cdot \frac{Vol(B_{kk'})}{m - \lvert J_{k-1}(> \tau_k) \rvert}.\]
Intuitively, the unblocked jobs are not problematic because there can be at most $m - \lvert J_{k-1}(> \tau_k) \rvert$ such jobs.

\begin{lem}\label{lem_unblocked}
    The unblocked jobs satisfy $\sum_k n/2^k \cdot \sum_{k' \leq k} \frac{Vol(U_{kk'})}{m - \lvert J_{k-1}(> \tau_k) \rvert} \leq \log n \cdot \sum_k n/2^k \cdot \tau_k$.   
\end{lem}
\begin{proof}
    Because there are $\log n$ batches, it suffices to show for fixed $k$ and $k'$ that $\frac{Vol(U_{kk'})}{m - \lvert J_{k-1}(> \tau_k) \rvert} \leq \tau_k$. We recall that every job in $U_{kk'}$ is $\tau_k$-small, so:
    \[\frac{Vol(U_{kk'})}{m - \lvert J_{k-1}(> \tau_k) \rvert} \leq \tau_k \cdot \frac{\lvert U_{kk'} \rvert}{m - \lvert J_{k-1}(> \tau_k) \rvert}.\]
    
    Note $m - \lvert J_{k-1}(> \tau_k) \rvert$ is exactly the number of machines that do not schedule any $\tau_k$-big job in $J_{k-1}$ in $Opt$ (because $Opt$ schedules at most one $\tau_k$-big job per machine in $J_{k-1} \subset J_k^*$.) Further, every job in $U_{kk'}$ is $\tau_{k'}$-big and $U_{kk'} \subset I_{k'}^*$. Thus, $Opt$ schedules at most one job in $U_{kk'}$ per such machine. We conclude, $\frac{\lvert U_{kk'} \rvert}{m - \lvert J^*_{k-1}(> \tau_k) \rvert} \leq 1$, as required.
\end{proof}

It remains to handle the blocked jobs. This is the central issue in the analysis of \choosealg: The blocked jobs are exactly those that $Opt$ does in an earlier batch before some machines get clogged. On the other hand, \choosealg puts these jobs in a later batch when we have fewer machines.

We will charge the volume of these jobs to the completion time of $Opt$. Because these jobs are blocked, $Opt$ must schedule a $\tau_k$-big job later on the same machine. In particular, $Opt$ must have kept scheduling Bernoulli jobs with size parameter at least $\tau_k$ until one comes up heads. We will charge $B_{kk'}$ to the completion time of all of these coin flips.

As before, we consider a fixed threshold $\tau$ and later union bound over all relevant thresholds. In this section, for any batch $k$ and threshold $\tau$, we define $p^*_{k \tau} \in [0,1]$ to be the largest probability parameter across all jobs $j$ in $J_{k-1}$ with $s_j > \tau$ (if no such job exists, then we follow the convention $p^*_{k \tau} = 0$.) Note that $p^*_{k \tau}$ is deterministic for fixed $\tau$. We first relate the number of remaining machines with the expected number of heads in the $k$th batch.

\begin{prop}\label{prop_blocked_num_delayed}
    Consider any batches $k$, $k' \leq k$ and threshold $\tau \geq 2 \mathbb{E} F^*(n-n/2^k)$. Suppose Event (\ref{event_delta_big}) holds. Then we have $m- J_{k-1}(> \tau) \geq p^*_{k \tau} \cdot n/2^k - O(\Delta)$, where $\Delta = O(\sqrt{m} \log n)$.
\end{prop}
\begin{proof}
    We may assume $p^*_{k \tau} > 0$ or else the proposition is trivial. In particular, \choosealg included at least one job $j \in J_{k-1}$ with $s_j > \tau$ and $p_j = p^*_{k \tau}$. It follows, \choosealg will include $n/2^k$ further jobs in $I_k$ with size parameter larger than $\tau_k$ and probability parameter at least $p^*_{k \tau}$. Thus, we have $\mathbb{E} \lvert I_k(> \tau) \rvert \geq p^*_{k \tau} \cdot n/2^k$. Rewriting $\mathbb{E} \lvert I_k(> \tau) \rvert = \mathbb{E} \lvert J_k(> \tau) \rvert - \mathbb{E} J_{k-1}(> \tau) \rvert$ and applying \Cref{lem_big_job_small_expectation} and Event (\ref{event_delta_big}) to the first and second expectations, respectively gives the desired result:
    \[p^*_{k \tau} \cdot n/2^k \leq \mathbb{E} \lvert I_k(> \tau) \rvert = \mathbb{E} \lvert J_k(> \tau) \rvert - \mathbb{E} J_{k-1}(> \tau) \rvert \leq m + O(\sqrt{m}) - \lvert J_{k-1}(> \tau) \rvert + O(\Delta).\]
\end{proof}

To see the utility of \Cref{prop_blocked_num_delayed}, we assume for a moment that $\tau_k$ is deterministic and ignore the additive $O(\Delta)$ term in the proposition. Then we could rewrite $n/2^k \cdot \frac{Vol(B_{kk'})}{m - \lvert J_{k-1}(> \tau_k) \rvert} \lesssim \frac{1}{p^*_{k \tau}} \cdot Vol(B_{kk'})$.

To relate this expression with $Opt$, we note that $Opt$ schedules a $\tau_k$-big job on top of each job in $B_{kk'}$. In particular, $Opt$ must schedule enough Bernoulli jobs $j$ with $s_j > \tau_k$ until at one comes up heads on each such machine. Each such job also satisfies $p_j \leq p^*_{k \tau_k}$, so - roughly - in $Opt$ we expect each blocked job to delay at least $\frac{1}{p^*_{k \tau}}$ jobs in order for that machine to become blocked. This would give $\frac{1}{p^*_{k \tau_k}} \cdot Vol(B_{kk'}) \lesssim \sum_j C_j^*$, as required.

It remains to formalize this idea using a martingale argument.  We begin by defining an (artificial) game, which will model the process of a machine becoming blocked.

\begin{definition}[Coin Game]\label{def_coin_game}
    The game is played with $n$ coins and $m$ machines by a single player. The coins are independent such that coin $j$ comes up heads with probability $p_j$. Initially, all machines are \emph{available}.
    
    At each turn, the player can either choose to flip a previously unflipped coin on an available machine or to end the game. In the former case, if the coin comes up heads, then the machine becomes unavailable.

    The game ends when the player chooses to, or if we run out of unflipped coins or available machines.
\end{definition}

Now we are ready to interpret $Opt$ in our completion time minimization problem as implicitly playing a coin game to block machines.

\begin{definition}[Induced Coin Game]\label{def_induced_coin_game}
    Consider pairs of batches $k' \leq k$ and thresholds $\tau' \leq \tau$. Let $Opt$ denote the optimal adaptive policy for completion time minimization. Then the $(k', k, \tau', \tau)$-induced coin game (with respect to policy $Opt$) is a distribution over coin games defined as follows:
    \begin{itemize}
        \item The machines are the ones of $Opt$ whose final job in $J_{k'}^*$ has size exactly $\tau'$.
        \item For every job in $j \in J_k \setminus J_{k'}^*$ with $s_j > \tau$, we have a coin with the same probability parameter.
    \end{itemize}
    The player of the coin game simulates $Opt$ as follows. Starting from after $Opt$ schedules $J_{k'}^*$, if $Opt$ subsequently schedules a job on a machine that is still available (in the coin game), then the player flips the corresponding coin on the same machine. The player decides to stop when it runs of out coins or all machines are unavailable. \alert{not sure if formal enough}
\end{definition}

One should imagine that the machines in the induced coin game are exactly those that can become blocked. Thus, a machine becoming unavailable in the coin game corresponds to it becoming blocked in $Opt$, and the total number of flipped coins records how many jobs were delayed by $\tau'$.

Using a martingale argument, we relate the number of machines that become unavailable with the number of flipped coins. The next lemma formalizes the idea that to block a machine, we `expect' $Opt$ to flip $\frac{1}{p_{k\tau_k}^*}$ coins. Recall that for any batch $k$ and threshold $\tau$, we define $p^*_{k\tau}$ to be the largest probability parameter across all jobs $j$ in $J_{k-1}$ with $s_j > \tau$.

\begin{lem}\label{lem_induced_coin_game_concentration}
    Suppose Event (\ref{event_delta_big}) holds. Then with probability $1 - \frac{1}{poly(n)}$, for all pairs of batches $k' \leq k$ and thresholds $\tau' \leq \tau$ with $\tau > 2 \mathbb{E} F^*(n - n /2^k)$ and $p_{k \tau}^* > 0$, the $(k', k, \tau', \tau)$- induced coin game satisfies:
    \begin{equation}\label{event_coin_cost}
        \#(\text{unavailable machines}) \leq p^*_{k\tau} \cdot \#(\text{flipped coins}) + \Delta,
    \end{equation}
    where $\Delta = O(\sqrt{m} \log n)$.
\end{lem}
\begin{proof}
    Because there are $O(\log n)$ batches and $L \leq n$ relevant thresholds, by union-bounding over all pairs of batches and thresholds, it suffices to show that a fixed $(k',k',\tau',\tau)$-induced coin game satisfies:
    \[\mathbb{P}(\#(\text{unavailable machines}) \leq p^*_{k\tau} \cdot \#(\text{flipped coins}) + \Delta) = 1 - \frac{1}{poly(n)}.\]
    We will define a martingale to count the number of unavailable machines. For all $t \geq 0$, let $A_t$ be the (adaptively chosen) set of the first $t$ coins flipped by the player. If the player stops before flipping $t$ coins, then we define $A_t = A_{t-1}$. Now consider the sequence of random variables $M_t = \sum_{j \in A_t} C_j - \sum_{j \in A_t} p_j$ for all $t \geq 0$, where $C_j \sim Ber(p_j)$ is the distribution of coin $j$. Note that $\sum_{j \in A_t} C_j$ is exactly the number of heads in the first $t$ coin flips, which is the number of unavaiable machines.
    
    We claim that $M_t$ is a martingale. Consider any $t \geq 0$. There are two cases. If $A_t = A_{t-1}$, then $M_t = M_{t-1}$, so trivially $\mathbb{E}[M_t \mid M_{t-1}, \dots, M_0] = M_{t-1}$. Otherwise, $A_t = A_{t-1} \cup \{j\}$ for some adaptively chosen coin $j$. It suffices to show the martingale property conditioned on the next coin being $j$ for any fixed coin $j$:
    \begin{align*}
       \mathbb{E}[M_t \mid M_{t-1}, \dots, M_0, A_t = A_{t-1} \cup \{j\}] &= \mathbb{E}[M_{t-1} + C_j - p_j\mid M_{t-1}, \dots, M_0, A_t = A_{t-1} \cup \{j\}]\\
       &= M_{t-1} + p_j - p_j = M_{t-1},
    \end{align*}
    as required.
    
    To bound the deviation of $M_t$, we apply Freedman's inequality to the martingale difference sequence of $M_t$.

    \begin{prop}[Freedman's Inequality]\label{prop_freedman}
        Consider a real-valued martingale sequence $\{X_t\}_{t \geq 0}$ such that $X_0 = 0$ and $\lvert X_t \rvert \leq M$ almost surely for all $t$. Let $Y_t = \sum_{s = 0}^t \mathbb{E}[X_s^2 \mid X_{s -1}, \dots, X_0]$ denote the quadratic variation process of $\{X_t\}_t$. Then for any $\ell \geq 0, \sigma^2 > 0$ and stopping time $\tau$, we have:
        \[\mathbb{P}(\lvert \sum_{t = 0}^\tau X_t \rvert \geq \ell \text{ and } Y_\tau \leq \sigma^2) \leq 2 \cdot \exp{(- \frac{\ell^2 / 2}{\sigma^2 + M \ell / 3})}.\]
    \end{prop}

    We let $X_t$ denote the martingale difference sequence of $M_t$, which is defined as $X_0 = 0$ and $X_t = M_t - M_{t-1}$ for all $t > 0$. Because $M_t$ is a martingale, $X_t$ is as well. Further, we have $\lvert X_t \rvert \leq  1$ almost surely for all $t$. For any $t \geq 0$, we let $j_t$ be the (adaptively chosen) $t$th coin flip. Then we can bound the quadratic variation process by:
    \begin{align*}
        Y_t = \sum_{s = 0}^t \mathbb{E}[X_s^2 \mid X_{s -1}, \dots, X_0] &= \sum_{s = 0}^t \mathbb{E}[(C_{j_s} - p_{j_s})^2 \mid X_{s-1}, \dots, X_0]\\
        &\leq \sum_{s = 0}^t \mathbb{E}[C_{j_s}^2 \mid X_{s-1}, \dots, X_0]\\
        &= \sum_{s = 0}^t \mathbb{E}[C_{j_s} \mid X_{s-1}, \dots, X_0].
    \end{align*}
    Note that the $C_{j_1} + \dots C_{j_t} \leq m$ almost surely, because the induced coin game has at most $m$ machines, and any adaptive policy can flip at most one heads per machine. Thus, we have $Y_t \leq m$ for all $t$.
    
    Now let $T$ be the stopping time when the induced coin game ends, so $T$ is exactly the number of flipped coins. Then Freedman's Inequality gives:
    \[\mathbb{P}(\lvert \sum_{t = 0}^T X_t \rvert \geq \Delta) = \mathbb{P}(\lvert \sum_{t = 0}^T X_t \rvert \geq \Delta \text{ and } Y_T \leq m) \leq 2 \cdot \exp(- \frac{\Delta^2/2}{m + \Delta/3}).\]
    Taking $\Delta = O(\sqrt{m} \log n)$ gives $\mathbb{P}(\lvert \sum_{t = 0}^T X_t \rvert \geq \Delta) \leq \frac{1}{poly(n)}$.
    
    Finally, we observe that $\#(\text{unavailable machines}) = \sum_{j \in A_T} C_j$. Further, we have $p^*_{k\tau} \cdot \#(\text{flipped coins}) \geq \sum_{j \in A_T} p_j$, because every coin $j$ corresponds to a job in $J_{k-1}$ with $s_j > \tau$, so $p_j \leq p_{k\tau}^*$ for all coins. Thus, we conclude:
    \[\mathbb{P}(\#(\text{unavailable machines}) > p_{k \tau}^* \cdot \#(\text{flipped coins}) + \Delta) \leq \mathbb{P}(\lvert \sum_{t = 0}^T X_t \rvert > \Delta) \leq \frac{1}{poly(n)}.\]
\end{proof}

Combining \Cref{prop_blocked_num_delayed} and \Cref{lem_induced_coin_game_concentration}, we can bound the blocked jobs:

\begin{lem}\label{lem_blocked}
    Suppose Events (\ref{event_delta_big}) and (\ref{event_coin_cost}) hold. Then the blocked jobs satisfy:
    \[\sum_k n/2^k \cdot \sum_{k' \leq k} \frac{Vol(B_{kk'})}{m - \lvert J_{k-1}(> \tau_k) \rvert} = O(\Delta \cdot \log^3 n) (\sum_k n/2^k \cdot \tau_k + \sum_j C_j^*),\]
    where $\Delta = O(\sqrt{m} \log n)$.
\end{lem}
\begin{proof}\alert{to check: delicate proof using definitions of blocked and the coin game}
    Because there are $O(\log n)$ batches $k$, it suffices to show for fixed $k, k' \leq k$ that $n/2^k \cdot \frac{Vol(B_{kk'})}{m - \lvert J_{k-1}(> \tau_k) \rvert} = O(\Delta \cdot \log n) ( n/2^k \cdot \tau_k + \sum_j C_j^*)$. We consider two cases.
    
    First, on the event that $p_{k\tau_k}^* = 0$, we have $m - \lvert J_{k-1}(> \tau_k) \rvert = m$. Recall that every job in $B_{kk'}$ is $\tau_{k'}$-big and in $I_{k'}^*$, so there is at most one such job per machine. Then we can bound:
    \[n/2^k \cdot \frac{Vol(B_{kk'})}{m - \lvert J_{k-1}(> \tau_k) \rvert} \leq n/2^k \cdot \tau_k \frac{m}{m} = n/2^k \cdot \tau_k.\]
    
    Otherwise, we have $p_{k\tau_k}^* > 0$. Here we related the blocked jobs to the induced coin games:
    \begin{align*}
        Vol(B_{kk'}) &= \sum_{\tau' \leq \tau_k} \tau' \cdot \lvert \{j \in B_{kk'} \mid X_j = \tau'\} \rvert\\
        &= \sum_{\tau' \leq \tau_k} \tau' \cdot \#(\text{unavailable machines in $(k',k, \tau', \tau_k)$-induced coin game})\\
        &\leq \sum_{\tau' \leq \tau_k} \tau' \cdot (p_{k\tau_k}^* \cdot \#(\text{flipped coins in $(k',k, \tau', \tau_k)$-induced coin game}) + \Delta)\\
        &\leq O(\log n) \cdot p_{k \tau_k}^* \sum_j C_j^* + O(\Delta \cdot \log n) \cdot \tau_k.
    \end{align*}
    where the first inequality follows from Event (\ref{event_coin_cost}). The second follows because there are $O(\log n)$ relevant thresholds $\tau' \leq \tau_k$, and every flipped coin in the $(k',k, \tau', \tau_k)$-induced coin game corresponds to $Opt$ scheduling a job on a machine that already scheduled some job with size $\tau'$, so every such job has completion time at least $\tau'$. It follows:
    \[n/2^k \cdot \frac{Vol(B_{kk'})}{m - \lvert J_{k-1}(> \tau_k) \rvert} \leq n/2^k \cdot O(\log n) \frac{p_{k\tau_k}^*}{m - \lvert J_{k-1}(> \tau_k) \rvert} \sum_j C_j^* + n/2^k \cdot O(\Delta \cdot \log n) \frac{\tau_k}{m - \lvert J_{k-1} \rvert}.\]
    By \Cref{prop_blocked_num_delayed}, we can bound the first term by:
    \[n/2^k \cdot O(\log n) \frac{p_{k\tau_k}^*}{m - \lvert J_{k-1}(> \tau_k) \rvert} \sum_j C_j^* \leq O(\log n) \frac{m - \lvert J_{k-1}(> \tau_k) \rvert + O(\Delta)}{m - \lvert J_{k-1}(> \tau_k) \rvert} \sum_j C_j^* = O(\Delta \cdot \log n) \sum_j C_j^*.\]
    We can bound the second term by:
    \[n/2^k \cdot O(\Delta \cdot \log n) \frac{\tau_k}{m - \lvert J_{k-1} \rvert} = O(\Delta \cdot \log n) \cdot n/2^k \cdot \tau_k.\]
    Combining both bounds completes the proof.
\end{proof}

We summarize our bounds for the unblocked- and blocked jobs by the next lemma, which follows immediately from \Cref{lem_unblocked} and \Cref{lem_blocked}.

\begin{lem}\label{lem_blocked_and_unblocked}
    Suppose Events (\ref{event_delta_big}) and (\ref{event_coin_cost}) hold. Then the big-in-the-past jobs satisfy:
    \[\sum_k n/2^k \cdot \sum_{k' \leq k} \frac{Vol(I_k \cap I_{k'}^*(> \tau_{k'}, \leq \tau_k))}{m - \lvert J_{k-1}(> \tau_k) \rvert} = O(\Delta \cdot \log^3 n) (\sum_k n/2^k \cdot \tau_k + \sum_j C_j^*),\]
    where $\Delta = O(\sqrt{m} \log n)$.
\end{lem}

\subsection{Putting it all together: Proof of \Cref{thm_batches_opt_cost}}

We complete the proof of \Cref{thm_batches_opt_cost} by combining our bounds for the small-in-the-past- and big-in-the-past jobs. We recall the expression we want to bound (in expectation):
\[\sum_k n/2^k \cdot \frac{Vol(I_k(\leq \tau_k))}{m - \lvert J_{k-1}(> \tau_k) \rvert} = \sum_k n/2^k \cdot \sum_{k' \leq k} \frac{Vol(I_k \cap I_{k'}^*(\leq \tau_{k'}))}{m - \lvert J_{k-1}(> \tau_k) \rvert} + \sum_k n/2^k \cdot \sum_{k' \leq k} \frac{Vol(I_k \cap I_{k'}^*(> \tau_{k'}, \leq \tau_k))}{m - \lvert J_{k-1}(> \tau_k) \rvert}.\]
On Events (\ref{event_delta_big}) and (\ref{event_coin_cost}), we can apply \Cref{lem_small_past} to the first term and \Cref{lem_blocked_and_unblocked} to obtain:
\[\sum_k n/2^k \cdot \frac{Vol(I_k(\leq \tau_k))}{m - \lvert J_{k-1}(> \tau_k) \rvert} = O(\Delta \cdot \log^3 n) (\sum_k n/2^k \cdot \tau_k + \sum_j C_j^*),\]
where $\Delta = O(\sqrt{m} \log n)$.

Now we consider the event that Event (\ref{event_delta_big}) or Event (\ref{event_coin_cost}) does not hold. Recall that by \Cref{lem_big_job_chernoff} and \Cref{lem_induced_coin_game_concentration}, this happens with probability at most $\frac{1}{poly(n)}$. Further, on this event, we can trivially upper bound $\sum_k n/2^k \cdot \frac{Vol(I_k(\leq \tau_k))}{m - \lvert J_{k-1}(> \tau_k) \rvert} = poly(n)$, because there are $n$ jobs each with size at most $poly(n)$ almost surely. Thus, the contribution of this event to the overall expectation is $O(1)$. \alert{should write some other rescaling argument to show $\mathbb{E} Opt = \Omega(1)$, but this should be trivial.}
